First-order mean-field games on networks and Wardrop equilibrium

Here, we examine the Wardrop equilibrium model on networks with flow-dependent costs and its connection with stationary mean-field games (MFG). In the first part of this paper, we present the Wardrop and the first-order MFG models on networks. Then, we show how to reformulate the MFG problem into a Wardrop problem and prove that the MFG solution is the Wardrop equilibrium for the corresponding Wardrop problem. Moreover, we prove that the solution of the MFG problem can be recovered using the solution to the associated Wardrop problem. Finally, we study the cost properties and the calibration of MFG with Wardrop travel cost problems. We describe a novel approach to the calibration of MFGs. Further, we show that even simple travel costs can give rise to non-monotone MFGs.

==> __latexindent_temp.tex <==
\section{Wardrop equilibrium models and mean-field games}
\label{sec:current cost}

%{\color{red}
%What is the goal of this section: introduce the setting of generalized wardrop equilibrium; explain how this setting can be converted into a directed network by doubling edges.
%Describe the inner product in a directed network.
%Explain monotonicity conditions.
%Define projection on affine subspace.variational formulation and optimality conditions}

Here, we discuss the connection between Wardrop equilibria and stationary (congestion) MFGs on networks.
Traditionally, the Wardrop equilibrium is formulated on a directed network.
In this network, agents seek to find the least costly path between entrances and exits.
In our Wardrop model, we consider the case where agents enter in a finite set of vertices with a prescribed current intensity and leave through a set of exit vertices where they pay an exit cost.
This problem is closely related to MFGs on networks, where the entry currents and the exit costs are similarly given.
However, in MFGs the network is not directed.
Thus, the direction of the current in each edge is not prescribed a priori.

We begin in Section \ref{Wmodel} with a discussion of the Wardrop equilibrium model and a uniqueness theorem.
Next, in Section \ref{1edgegrapgh} we present the MFG model in a single edge.
Then, in Section \ref{MFG model} we generalize our work to include the MFG model on a network.
Finally, in Sections \ref{MFGtoW} and \ref{WtoMFg} we make the connection between the MFGs and the Wardrop model.
%by reformulating the MFG into a Wardrop model.


\subsection{Wardrop equilibrium model}\label{Wmodel}

We consider a steady-state model of agents traveling through a network with flow dependent travel costs on the edges.
Following the presentation of the model's elements, we discuss an equilibrium concept due to Wardrop \cite{Wardrop52}. Later, in Subsection \ref{MFGtoW}, we show how this concept is related to the MFG model presented in Subsection \ref{MFG model}.
This model consists of the following:
\begin{enumerate}
\item A finite \textbf{directed} network (graph), $\tilde{\Gamma}=(\tilde{E},\tilde{V})$, where
$\tilde{E} = \{ \tilde{e}_k : k \in \{1,2,\dots,\tilde{n}\} \}$ is the set of edges
and $\tilde{V}=\{\tilde{v}_i : i \in \{1,2,\dots, \tilde{m}\} \}$ is the set of vertices.
To any edge $\tilde{e}_k$ we associate the pair $(\tilde{v}_r,\tilde{v}_i)$ of its endpoints, which maybe identified with $\tilde{e}_k$ if there is no ambiguity. 
%We write $\tilde{e}_k=(\tilde{v}_r,\tilde{v}_i)$ for the directed edge from $\tilde{v}_r$ to $\tilde{v}_i$.


\item The \emph{current} or the flow is the number of agents crossing a given point per unit of time.
The current in the edge $\tilde{e}_k$ is denoted by $\tilde{\jmath}_k$.

The current on the network is the $\tilde{n}$-dimensional vector $\bm{\tilde{\jmath}}=(\tilde{\jmath}_1,\dots,\tilde{\jmath}_{{\tilde{n}}})$.


\item The \emph{travel cost} in each edge $\tilde{e}_k$ is given by a function $ {\tilde{c}}_k : \tilde{E} \rightarrow \mathbb{R}$.
%in each edge $\tilde{e}_k$ is given by the function $\tilde{c}_k(\bm{\tilde{\jmath}})$.
The cost is local if $ {\tilde{c}}_k$ depends only on $\tilde{\jmath}_k$.
%The cost may be local; that is, depends only on $\tilde{\jmath}_k$, or be non local; that is, depends on the whole vector $\bm{\tilde{\jmath}}$.
%The cost in the auxiliary exit edges is zero.

We denote the vector of the costs in the edges by $\bm{\tilde{c}}(\bm{\tilde{\jmath}})=(\tilde{c}_1(\bm{\tilde{\jmath}}),\dots,\tilde{c}_{\tilde{n}}(\bm{\tilde{\jmath}}))$. Observe that 
$\langle\bm{\tilde{c}}(\bm{\jmath}),\bm{\jmath}\rangle:= \sum_{k=1}^{\tilde{n}} \tilde{c}_k(\bm{\jmath})j_k $ is the social cost per unit of time corresponding to the distribution of currents $\bm{\jmath}$.




\item  Agents enter the network through $\tilde{\lambda}$ {\em entrance vertices}. A flow of agents, the entry current $\tilde{\bm{\iota}}=(\tilde{{\iota}}_1,\dots,\tilde{{\iota}}_{\tilde{\lambda}}) >0$, is prescribed at the entrance vertices.
The entry currents in the other vertices are zero.
This information is encoded in the $(\tilde{m}-\tilde{l})$-dimensional vector $\tilde{B}$.

\item Agents exit the network through $\tilde{l}$
{\em exit vertices} (disjoint from the entrance vertices). 
For convenience, we assume that the last $\tilde{l}$ vertices in $\tilde{V}$ are the exit vertices. 
At the $\tilde{l}$ exit vertices, agents pay an exit cost $\tilde{\bm{\psi}}$. Here, we assume that this exit cost vanishes. 
Furthermore, we suppose that the incidence of exit vertices is $1$.
As discussed in the remark below this assumption entails no loss of generality. 
\end{enumerate}
\begin{remark}
If a vertex with an incidence of more than $1$ is labeled as an exit, we can attach an auxiliary exit edge to it, relabeling its extra vertex as the new exit vertex.
In the  auxiliary exit edge the travel cost is the exit cost and at the  new exit vertex the exit cost is zero.  
\end{remark}

Let $\tilde{K}$ be the $(\tilde{m}-\tilde{l}) \times \tilde{n}$ Kirchhoff matrix, obtained by removing $\tilde{l}$ lines corresponding to the exit vertices of $\tilde{\Gamma}$ from the \emph{incidence matrix} of $\tilde{\Gamma}$, i.e.,
\begin{equation}\label{K}
\tilde{K}_{ik}=
\begin{cases}
1 \ \ \text{if} \ \tilde{e}_k=(\tilde{v}_i,\tilde{v}_r) \\
-1\ \ \text{if} \ \tilde{e}_k=(\tilde{v}_r,\tilde{v}_i)\\
0 \ \ \text{if} \ \tilde{v}_i \not\in \tilde{e}_k,
\end{cases}
\end{equation}
%1 \ \ \text{if} \ \tilde{e}_k \ \text{goes out of} \ \tilde{v}_i \\
%-1\ \ \text{if} \ \tilde{e}_k \ \text{goes into} \ \tilde{v}_i \\
%0 \ \ \text{if} \ \tilde{e}_k \ \text{is not incident to} \ \tilde{v}_i,
where $ i \in \{1,2,\dots, \tilde{m}-\tilde{l}\}$ and $k \in \{1,2,\dots,\tilde{n}\} $.
The rows in $\tilde{K}$ correspond to non-exit vertices of the network, and the columns correspond to the edges. 
% For convenience, we assume that the last $\tilde{l}$ vertices are exit vertices. 
\begin{definition}
A distribution of currents, ${\bm{\tilde{\jmath}}} \geq 0$, is \emph{admissible} if 
\begin{equation}\label{admis}
\tilde{K}\bm{\tilde{\jmath}}=\tilde{B}.
\end{equation}
The set of all admissible distributions of currents is denoted by $\mathcal{A}$.
\end{definition}
\begin{remark}
The $\tilde{m}-\tilde{l}$ equations in \eqref{admis} correspond to  Kirchhoff's law for the non-exit vertices.
\end{remark}

Next, following Smith (\cite{Smith1979traffic}), we define the Wardrop equilibrium.
\begin{definition}\label{defWard}
A distribution of currents ${\bm{\tilde{\jmath}}}^* \in \mathcal{A}$ is a \emph{ Wardrop equilibrium} if, for all $\bm{\tilde{\jmath}} \in \mathcal{A}$,
\begin{equation}\label{Wardrop}
\langle \bm{\tilde{c}}({\bm{\tilde{\jmath}}}^*),{\bm{\tilde{\jmath}}}^*-\bm{\tilde{\jmath}} \rangle \leq 0.
\end{equation}
\end{definition}
In Section \ref{WtoMFg}, we prove that Definition \ref{defWard} means that in Wardrop equilibrium, any current-carrying path is optimal in the sense that it minimizes the travel cost to the exit. 
%no agent has a unilateral incentive to change its strategy.

% \paragraph{Uniqueness of Wardrop equilibria.}
We use the notion of monotonicity, defined below, to state and prove a result on the uniqueness of Wardrop equilibria.
\begin{definition}
A cost $\bm{\tilde{c}}$ is \emph{monotone} if, for any $\bm{\tilde{\jmath}_1}, \bm{\tilde{\jmath}_2} \in \mathcal{A}$,
\begin{equation}\label{mono}
\langle \bm{\tilde{c}}(\bm{\tilde{\jmath}_1})-\bm{\tilde{c}}(\bm{\tilde{\jmath}_2}),\bm{\tilde{\jmath}_1}-\bm{\tilde{\jmath}_2} \rangle \geq 0.
\end{equation}
If, for $\bm{\tilde{\jmath}_1} \neq \bm{\tilde{\jmath}_2}$, the inequality in \eqref{mono} is strict, then we say that $\bm{\tilde{c}}$ is \emph{strictly monotone}.
\end{definition}
\begin{example}
If $\tilde{c}_k$ depends only on $\tilde{\jmath}_k$ and is increasing, %in $\tilde{\jmath}_k$,
then $\bm{\tilde{c}}$ is monotone.
\end{example}
Strict monotonicity of the cost is sufficient for uniqueness.
\begin{theorem}[Uniqueness of Wardrop equilibrium]
If the cost $\bm{\tilde{c}}$ is strictly monotone on the set $\mathcal{A}$.
Then, there is at most one Wardrop equilibrium.
\end{theorem}
\begin{proof}
Suppose ${\bm{\tilde{\jmath}_1}}$ and ${\bm{\tilde{\jmath}_2}}$ are Wardrop equilibria.
Then, for any $\bm{\tilde{\jmath}} \in \mathcal{A}$, we have
\begin{equation}
\langle \bm{\tilde{c}}({\bm{\tilde{\jmath}_1}}),{\bm{\tilde{\jmath}_1}}-\bm{\tilde{\jmath}} \rangle \leq 0
\ \text{and} \
\langle \bm{\tilde{c}}({\bm{\tilde{\jmath}_2}}),{\bm{\tilde{\jmath}_2}}-\bm{\tilde{\jmath}} \rangle \leq 0.
\end{equation}
Accordingly,
$$
\langle \bm{\tilde{c}}({\bm{\tilde{\jmath}_1}})-\bm{\tilde{c}}({\bm{\tilde{\jmath}_2}}),{\bm{\tilde{\jmath}_1}}-{\bm{\tilde{\jmath}_2}} \rangle \leq 0,
$$
and because $\bm{\tilde{c}}$ is strictly monotone, ${\bm{\tilde{\jmath}_1}}={\bm{\tilde{\jmath}_2}}$.
\end{proof}

Next, we discuss a necessary condition for the existence of a Wardrop equilibrium.
%For this, we recall that
\begin{definition}
A current distribution $\bm{\tilde{\jmath}_0} \geq 0$ on $\Gamma$ is a \emph{current loop} if it is a nontrivial solution of $\tilde{K}\bm{\tilde{\jmath}_0}=0$.
\end{definition}

\begin{proposition}\label{loopcost}
If $\bm{\tilde{\jmath}^*}$ is a Wardrop equilibrium, then
$$
\langle \bm{\tilde{c}}(\bm{\tilde{\jmath}^*}),\bm{\tilde{\jmath}_0} \rangle \geq 0,
$$
for any current loop, $\bm{\tilde{\jmath}_0}$.
\end{proposition}
\begin{proof}
Let $\bm{\tilde{\jmath}^*}$ be the Wardrop equilibrium and let
$$
\bm{\tilde{\jmath}}(\varepsilon)=\bm{\tilde{\jmath}^*}+\varepsilon \bm{\tilde{\jmath}_0}.
$$
Since $\bm{\tilde{\jmath}_0}$ is a non-trivial loop, $\bm{\tilde{\jmath}}(\varepsilon) \in \mathcal{A}$, for $\varepsilon \in \mathbb{R}^+_0$.
Condition \eqref{Wardrop} for the particular $\bm{\tilde{\jmath}}(\varepsilon)$ implies that
$$
\langle \bm{\tilde{c}}(\bm{\tilde{\jmath}^*}),\bm{\tilde{\jmath}^*}-(\bm{\tilde{\jmath}^*}+\varepsilon \bm{\tilde{\jmath}_0}) \rangle =
-\varepsilon \langle \bm{\tilde{c}}(\bm{\tilde{\jmath}^*}),\bm{\tilde{\jmath}_0} \rangle \leq 0, \ \forall \varepsilon >0.
$$
Thus,
$
\langle \bm{\tilde{c}}(\bm{\tilde{\jmath}^*}),\bm{\tilde{\jmath}_0} \rangle \geq 0.
$
\end{proof}
\begin{remark}
Proposition \ref{loopcost} states that any edge that admits a positive current in a current loop has a non-negative cost in the Wardrop equilibrium.
%means that all current loops have non-negative costs.
%This is %a necessary condition for the existence of the solutions.
%For example, if all costs are positive, this condition is satisfied.
\end{remark}

Next, we examine the structure of Wardrop equilibrium in a specific case relevant to MFGs.
The networks arising in MFGs are undirected networks which can be transformed into directed networks by doubling the edges {\color{red}giving a direction to the edges and adding their reverses}.
Thus, these networks have as a basic building block the loop network in Figure \ref{loop}.
\begin{IMG}
{"loop",Graph[{Labeled[1 \[DirectedEdge] 2, Subscript[OverTilde["e"], k]],
Labeled[2 \[DirectedEdge] 1, Subscript[OverTilde["e"], l]]},
VertexLabels -> {1 -> Subscript[OverTilde["v"], r],
2 -> Subscript[OverTilde["v"], i]}, GraphLayout -> "RadialDrawing"](*\]\]*)}	
\end{IMG}
\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/loop.pdf}
\caption{Loop network.}
\label{loop}
\end{figure}
\begin{proposition}
Consider a network containing the edge
$\tilde{e}_k=(\tilde{v}_r,\tilde{v}_i)$ and the reverse edge $\tilde{e}_l=(\tilde{v}_i,\tilde{v}_r)$.
Let $\tilde{\jmath}_k \geq 0$ be the current in $\tilde{e}_k$, and $\tilde{\jmath}_l \geq 0$ be the current in $\tilde{e}_l$.
Let $\tilde{c}_k(\bm{\tilde{\jmath}})$ be the cost in $\tilde{e}_k$, and $\tilde{c}_l(\bm{\tilde{\jmath}})$ be the cost in $\tilde{e}_l$,
where $\bm{\tilde{\jmath}}=(\tilde{\jmath}_k,\tilde{\jmath}_l)$.
If the costs $\tilde{c}_k$ and $\tilde{c}_l$ satisfy the following condition,
\begin{equation}\label{poscost}
\tilde{c}_k(\bm{\tilde{\jmath}})+\tilde{c}_l(\bm{\tilde{\jmath}}) >0,
\end{equation}
then any Wardrop equilibrium ${\bm{\tilde{\jmath}}}^*=(\tilde{\jmath}^*_k,\tilde{\jmath}^*_l)$ satisfies the complementary condition
\begin{equation}\label{WardComp}
\tilde{\jmath}^*_k \cdot \tilde{\jmath}^*_l = 0, \ \ k\neq l.
\end{equation}
\end{proposition}
\begin{proof}
We prove the theorem for a network that has Figure \ref{loop} as a subnetwork.
Assume that ${\bm{\tilde{\jmath}}}^*=(\tilde{\jmath}^*_k,\tilde{\jmath}^*_l)$ is a Wardrop equilibrium and does not satisfy \eqref{WardComp}, i.e.,
without loss of generality $\tilde{\jmath}^*_k > \tilde{\jmath}^*_l > 0$.
Take $\bm{\tilde{\jmath}_0}=(\tilde{\jmath}^*_k-\tilde{\jmath}^*_l,0)$, then by \eqref{Wardrop}, we have
\begin{equation*}
\langle (\tilde{c}_k({\bm{\tilde{\jmath}}}^*),\tilde{c}_l({\bm{\tilde{\jmath}}}^*)), (\tilde{\jmath}^*_l,\tilde{\jmath}^*_l) \rangle \leq 0
\end{equation*}
which contradicts the assumption \eqref{poscost}.
Hence, ${\bm{\tilde{\jmath}}}^*$ cannot be a Wardrop equilibrium.
\end{proof}

%\begin{example}
%Consider the network in Figure \ref{loop}.
%Let $\tilde{v}_1$ be an entrance and $\tilde{v}_2$ be an exit.
%Let $\tilde{\jmath}_1$ be the current in $\tilde{e}_1$, and $\tilde{\jmath}_2$ be the current in $\tilde{e}_2$.
%Let $\tilde{c}_1(\bm{\tilde{\jmath}})$ be the cost in $\tilde{e}_1$, and $\tilde{c}_2(\bm{\tilde{\jmath}})$ be the cost in $\tilde{e}_2$,
%where $\bm{\tilde{\jmath}}=(\tilde{\jmath}_1,\tilde{\jmath}_2)$.
%Assume that the costs satisfy \eqref{poscost}.
%We show that if $\tilde{\jmath}_1$ and $\tilde{\jmath}_2$ do not satisfy the complementary condition \eqref{WardComp}, then $\bm{\tilde{\jmath}}$ is not a Wardrop equilibrium.
%To prove this, let $\tilde{\jmath}_1 >\tilde{\jmath}_2>0$ and ${\bm{\tilde{\jmath}}}^*=(\tilde{\jmath}_1,\tilde{\jmath}_2)$ be a Wardrop equilibrium, i.e.
%it satisfies \eqref{Wardrop}.
%Take $\bm{\tilde{\jmath}}=(\tilde{\jmath}_1-\tilde{\jmath}_2,0)$, then by \eqref{Wardrop}, we have
%\begin{equation*}
%\langle (\tilde{c}_1({\bm{\tilde{\jmath}}}^*),\tilde{c}_2({\bm{\tilde{\jmath}}}^*)), (\tilde{\jmath}_2,\tilde{\jmath}_2) \rangle \leq 0,
%\end{equation*}
%but this contradicts the assumption \eqref{poscost}.
%Hence, ${\bm{\tilde{\jmath}}}^*$ is not a Wardrop equilibrium.
%\end{example}

Next we analyze the monotonicity of the cost on a network containing the subnetwork in Figure \ref{loop}.
\begin{example}\label{exmono}
The monotonicity condition for the subnetwork in Figure \ref{loop} is
$$
\langle (\tilde{c}_1(\bm{\tilde{\jmath}}),\tilde{c}_2(\bm{\tilde{\jmath}}))-(\tilde{c}_1(\bm{\hat{\jmath}}),\tilde{c}_2(\bm{\hat{\jmath}})), \bm{\tilde{\jmath}}-\bm{\hat{\jmath}} \rangle \geq 0,
$$
where $\bm{\tilde{\jmath}}=(\tilde{\jmath}_1,\tilde{\jmath}_2)$ and $\bm{\hat{\jmath}}=({\hat{\jmath}}_1,{\hat{\jmath}}_2)$.
Then, we get
$$
(\tilde{c}_1(\bm{\tilde{\jmath}}) -\tilde{c}_1(\bm{\hat{\jmath}}), \tilde{\jmath}_1-\hat{\jmath}_1 )
+ ( \tilde{c}_2(\bm{\tilde{\jmath}}) -\tilde{c}_2(\bm{\hat{\jmath}}), \tilde{\jmath}_2-\hat{\jmath}_2 )
\geq 0.
$$
Suppose that
$\tilde{c}_1(\bm{\tilde{\jmath}})= \hat{c}_1(\tilde{\jmath}_1 - \tilde{\jmath}_2)$ and $\tilde{c}_2(\bm{\tilde{\jmath}})= \hat{c}_2(\tilde{\jmath}_2 - \tilde{\jmath}_1)$.
Then, we have
\begin{equation*}
(\hat{c}_1(\tilde{\jmath}_1 - \tilde{\jmath}_2)-
\hat{c}_1(\hat{\jmath}_1 - \hat{\jmath}_2),
\tilde{\jmath}_1-\hat{\jmath}_1) +
(\hat{c}_2(\tilde{\jmath}_2 - \tilde{\jmath}_1)-
\hat{c}_2(\hat{\jmath}_2 - \hat{\jmath}_1),
\tilde{\jmath}_2-\hat{\jmath}_2) \geq 0.
\end{equation*}
\end{example}

The previous example can be generalized to networks which are built out of subnetworks like the one in Figure \ref{loop}.
% We call this \emph{pairwise monotonicity} and write
The sum in the monotonicity condition
$$
\sum_k (\tilde{c}_k({\bm{\tilde{\jmath}}})-\tilde{c}_k({\bm{\hat{\jmath}}}))(
{\tilde{\jmath}}_k-{\hat{\jmath}}_k) \geq 0,
$$
can be organized in related pairs of edges.
If the cost is restricted to each of these pairs is monotone we say that the cost is \emph{pairwise monotone}.
We consider two cases of interest of pairwise monotonicity:
\begin{enumerate}
\item The constant costs.
Since they do not depend on the currents, we have
$$
\sum_k (\tilde{c}_k({\bm{\tilde{\jmath}}})-\tilde{c}_k({\bm{\hat{\jmath}}}),
{\bm{\tilde{\jmath}}}-{\bm{\hat{\jmath}}}) = 0.
$$
\item The costs arising from an MFG, which we discuss in Section \ref{MFGtoW}.
\end{enumerate}



%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%



\subsection{MFG problem in a single edge}\label{costsection}
Here, we begin our analysis of travel costs on networks in the context of MFGs. 
We start this discussion with the analysis of a single edge.
%Now, we study the MFG problem and the travel cost in a single edge.
%In the next section, we generalize the discussion to include networks.
\subsubsection{MFG system in an edge}
Consider an edge which is identified with the interval $[0,1]$. In this edge, we have a Hamiltonian $H:[0,1]\times \mathbb{R}\times\mathbb{R}_0^+\to \mathbb{R}$ which we assume to be a smooth function, convex in the second variable. 
The two unknowns that determine the MFG are the player's density $m:[0,1]\to \mathbb{R}_0^+$ and value function $u:[0,1]\to\mathbb{R}$. These two functions solve the MFG
% (for simplicity, we omit the dependence of $u$, $m$, and $j$ in the edge index $k$)
\begin{equation}\label{MFGgeneral}
\begin{cases}
H\left(x,u_x(x),m(x)\right)=0 \\
\left(-m(x)D_pH(x,u_x(x),m(x)\right)_x=0.
\end{cases}
\end{equation}
The first equation is the Hamilton-Jacobi (HJ) equation and the second is the transport equation.

From the second equation in \eqref{MFGgeneral}, the current 
\begin{equation}\label{ABC}
    j=-mD_pH\left(x,u_x(x),m(x)\right)
\end{equation} is constant along the edge.
Thus, in principle, we can solve \eqref{ABC} for $u_x$ and replace it in the first equation.
Accordingly, we obtain an algebraic equation for $m$, see Proposition {\color{red}3.20} for details. 
This equation defines a distribution of players $m(x,j)$. 
This procedure is known as the current method introduced in \cite{GNPr216}.
%This system is supplemented by boundary conditions which we discuss below.

Next, we present a family of Hamiltonians that are prototype for MFG congestion models, and illustrate this method. 
\begin{example}\label{ExampleMFG}
Let
$$
H(x,p,m)=\frac{|p|^2}{2m^{\alpha}} + V(x) - g(m),
$$
where $g$ is an increasing function, $V$ is a smooth function and $0\leq \alpha \leq 2$ is the congestion strength.
Then, \eqref{MFGgeneral} becomes
\begin{equation}\label{mfgs}
\begin{cases}
\frac{|u_x|^2}{2m^{\alpha}} + V(x) = g(m)\\
(-m^{1-\alpha}u_x)_x=0.
\end{cases}
\end{equation}
There are two special values of the parameter $\alpha$,
$\alpha=0$ for the uncongested MFG, and $\alpha=1$, corresponds to the critical congestion model, for which the system decouples.
In this last case, $u$ is a linear function and $m$ can be obtained by solving directly the first equation in \eqref{mfgs}.

Because the current, $j=-m^{1-\alpha}u_x$, is constant, we transform the MFG system \eqref{mfgs}, into the following algebraic system %for $j>0$
\begin{equation}\label{current mfg}
\begin{cases}
\frac{j^2}{2m^{2-{\alpha}}}+V(x)=g(m)\\
j\int_0^1m^{\alpha-1}dx=u(0)-u(1),\\
\end{cases}
\end{equation}
provided $m>0$.
We refer to the last equation in \eqref{current mfg} as the \emph{edge equation}.
In this equation, either $u(0)$ or $u(1)$ is given by boundary conditions.
The sign of the current indicates the direction in which the agents travel, from $0$ to $1$ when $j>0$ and from $1$ to $0$ when $j<0$.
When $j>0$, the edge equation determines $u(0)$ as a function of $u(1)$, whereas when $j<0$, this equation determines $u(1)$ as a function of $u(0)$.
This depends on how boundary conditions are specified as we discuss next.
\end{example}

\subsubsection{Travel cost in an edge}

Consider an edge and, as before, assume that this edge is identified with the interval $[0,1]$ and the vertices with $\{0,1\}$.
%Given a current $j$ on this edge we define the two travel costs between the vertices $c_{01}$ and $c_{10}$. 
Given the current $j$ in this edge, there are two costs.
The cost of moving from left to right, (i.e.
from $0$ to $1$), and it is denoted by $c_{01}(j)$, and the cost of moving from right to left, (i.e.
from $1$ to $0$), and it is denoted by $c_{10}(j)$.
To define these costs, we introduce the Lagrangian
\begin{equation*}
    L(x,v,m) =\sup_{p}{-p v -H(x,p,m)}.
\end{equation*}


\begin{definition}
Given a distribution of players $m(x,j)$,
the optimal cost of traveling from $0$ to $1$ on the edge, is 
% with a trajectory $x(t,j):[0,T] \rightarrow [0,1]$, is
\begin{equation}\label{costdef}
c_{01}(j)= \min_{\substack{x,T \\ x(0)=0\\ x(T)=1}}
\int_0^T L(x,\dot{x},m(x,j)) dt,
\end{equation}
where the minimum is taken over all Lipschitz trajectories and all possible terminal times.
The cost $c_{10}$ is defined analogously.
\end{definition}

The agent at a vertex of an edge has two options either leaving this edge or staying in the edge and cross it to get to the opposite vertex. This is encoded in the following inequalities
\begin{equation}\label{optforc}
\begin{cases}
u(1)\leq c_{10}(j)+u(0), \\
u(0)\leq c_{01}(j)+u(1).
\end{cases}
\end{equation}
%When the current is zero, we do not have equalities just inequalities.
Moreover, the self-consistency in MFGs requires that the direction in which the agent moves is aligned with the direction of the current.
This is reflected in the following condition
%From the discussion in Example \ref{ExampleMFG}, the boundary conditions in the MFG have to be consistent with the current in the edge in the following way
\begin{equation}\label{BC}
\begin{cases}
j>0 \Rightarrow u(0)=c_{01}(j)+u(1), \\
j<0 \Rightarrow u(1)=c_{10}(j)+u(0).
\end{cases}
\end{equation}

\begin{remark}
The optimality conditions in \eqref{optforc} imply the following local compatibility condition
$$
-c_{01}(j) \leq c_{10}(j).
$$
This can be interpreted as loops having a positive cost
$$
c_{01}(j)+c_{10}(j) \geq 0.
$$
\end{remark}
\begin{proposition}
If the costs in \eqref{optforc} are positive, then the inequalities in \eqref{optforc} are redundant.
% and there is a compact way to write this.
\end{proposition}
\begin{proof}
The optimality conditions \eqref{optforc} imply,
$$
-c_{01}(j) \leq u(1)-u(0) \leq c_{10}(j).
$$
If $j \neq 0$, one of the two inequalities is an equality.
Since the costs are positive, then the other inequality holds.
\end{proof}
%If the cost is allowed to be negative this can cause existence issues.

%Because MFGs are not given with an explicit cost function, we show next how to define the cost in the edge, in order to use it later in transferring the MFG problem into a Wardrop equilibrium problem.
Now, we analyze in detail, the variational problem that defines the cost. 

%The optimal cost of traveling from $0$ to $1$ with a trajectory $x(t,j):[0,T] \rightarrow [0,1]$, is
%$$
%c_{01}(j)= \min_{\substack{x\\ x(0)=0\\ x(T)=1}}
%\int_0^T L(x,\dot{x},m(x,j)) dt,
%$$
Parametrizing in \eqref{costdef} the velocity $v$ by the space coordinate $x$, so
$dx=v dt$
provided $\dot{x}>0$,
we get
\begin{equation}\label{Lv}
c_{01}(j)= \min_{v>0} \int_0^1 {\frac{L(x,v(x,j),m(x,j))}{v(x,j)}} dx.
\end{equation}
\begin{proposition}
    If $L(x,v,m)$ is coercive and $L(x,0,m)>0$, then there exists a function $v>0$ minimizing \eqref{Lv} and solving the Euler-Lagrange equation
    \begin{equation}\label{L/v}
        -\frac{L(x,v(x,j),m(x,j))}{v(x,j)^2}+\frac{D_vL(x,v(x,j),m(x,j))}{v(x,j)}=0.
        \end{equation}
    Moreover, if $L(x,v,m)$ is strictly convex, then $v$ is unique.
    \end{proposition}
    \begin{proof}
 %   The condition \eqref{L/v} is the necessary optimality condition for $v$ to minimize
  %  $$\int_0^1 \frac{L(x,v(x,j),m(x,j))}{v(x,j)} dx.$$
    Because $L(x,0,m(x,j))>0$, we have
    $$ \lim_{v \rightarrow 0} \frac{L(x,v(x,j),m(x,j))}{v(x,j)}= +\infty,$$
    and by coercivity, we have
    $$ \lim_{v \rightarrow \infty} \frac{L(x,v(x,j),m(x,j))}{v(x,j)}= +\infty.$$
    Then, there exists a minimizer $v>0$. This minimizer solves \eqref{L/v}.
    Uniqueness of $v$ follows from that
    $D^2_{vv}L(x,v,m) >0 $ for $v>0$, and that $L(x,0,m)>0$.
    {\color{red}(more details).}
    \end{proof}
    
    %(we may need $L(x,0,m)>0$ to prevent $v(x)=0$ )
%We minimize to find the optimal control $v$, (for $v>0$ it may be that the infimum is achieved for $v=0$), 


Let $v^*$ be a minimizer of \eqref{Lv}.
By \eqref{L/v}, we have 
\begin{equation}\label{DvL}
D_vL(x,v^*(x,j),m(x,j))=\frac{L(x,v^*(x,j),m(x,j))}{v^*(x,j)}.
\end{equation}
Thus,
\begin{equation}\label{cost}
c_{01}(j)= \int_0^1 {D_vL(x,v^*(x,j),m(x,j))} dx.
\end{equation}
Note that, $c_{01}$ is defined for any $j \in \mathbb{R}$. In particular, when $j<0$, $c_{01}$ is the best possible cost of moving against the current. 
% we can do when traveling possibly in the wrong direction, which corresponds to the case $j<0$.
Similarly, the optimal cost for traveling from $1$ to $0$ is
\begin{equation}\label{cost10}
c_{10}(j)= - \int_0^1 {D_vL(x,v^*(x,j),m(x,j))} dx.
\end{equation}

{\color{red} Explain: The optimal velocity for an agent traveling from 1 to 0 is\dots}

%%%%%%%%%%%%%%%%


Now, we examine the relation between the cost function and the value function. 


\begin{proposition}
    
        The cost $c_{01}(x,j)$ solves the MFG system
        \begin{equation}\label{mfgsys}
        \begin{cases}
        H(x,-c_{01}(x,j),m)=0, \\
        -mD_pH(x,-c_{01}(x,j),m)=j.
        \end{cases}
        \end{equation}
        
         For $j>0$, the cost  $c_{01}(j)$ is given by
  $$
  c_{01}(j)= \int_0^1  c_{01}(x,j) dx, 
  $$
   where
    $c_{01}(x,j)= -u_x$.
 
 Similarly, for $j<0$, the cost  $c_{10}(j)$ is given by
  $$
  c_{10}(j)= \int_0^1 c_{10}(x,j) dx,
  $$
  where $ c_{10}(x,j)= u_x$.
\end{proposition}
\begin{proof}
Consider an edge with a current, $j>0$.
%For definiteness, we consider the case $j>0$.
%This means that $u$ has a Dirichlet boundary condition to the right (at 1).
By the fundamental theorem of calculus,
$$
u(0)=u(1)-\int_0^1{u_x} dx.
$$
By the first identity in \eqref{BC}, we have 
$$
u(0)=u(1)+c_{01}(j). 
$$
Hence, 
$$
c_{01}(j)=-\int_0^1{u_x} dx.
$$
Thus, $-u_x$ can be regarded as a cost per unit of length.
We define $c_{01}(x,j) = -u_x$.
Therefore,
$$
c_{01}(j)=\int_0^1 c_{01}(x,j) dx.
$$
The proof of the case $j<0$, is similar. 
%this means that $u(0)$ is given.
%Following the same steps, we get
%$$
%u(1)=u(0)+ c_{10}(j).
%$$
\end{proof}

\begin{remark}
The cost $c_{01}(x,j)$ solves the MFG system
\begin{equation}\label{mfgsys}
\begin{cases}
H(x,-c_{01}(x,j),m)=0, \\
-mD_pH(x,-c_{01}(x,j),m)=j.
\end{cases}
\end{equation}
\end{remark}

\begin{proposition}
   
 
   If $H$ is strictly convex in $p$ then, we have the following 
    \begin{itemize}
   \item $ u_x=-D_vL\left(x,\frac{j}{m},m\right)$;
   \item   $m(x,j)$ solves 
\begin{equation}\label{m}
H\left(x,-D_vL\left(x,\frac{j}{m},m\right),m\right)=0.
\end{equation}

    \end{itemize}
\end{proposition}



\begin{proof}
Since $H$ is strictly convex in $p$, 
$ p \rightarrow D_pH(x,p,m)$
is invertible.
Moreover, if $D_vL(x,v,m)=-p$, $v=-D_pH(x,p,m)$, we have
\begin{equation}\label{p}
p=-D_vL(x,-D_pH(x,p,m),m).
\end{equation}
From the second equation in \eqref{mfgsys}, we have
$$
D_pH(x,u_x,m)=-\frac{j}{m}.
$$
Accordingly, we get
\begin{equation}\label{ux}
p=u_x=-D_vL(x,\frac{j}{m},m).
\end{equation}
Using \eqref{ux} in the HJ equation in \eqref{MFGgeneral}, we obtain
\begin{equation}\label{m}
H(x,-D_vL\left(\left(x,\frac{j}{m},m\right),m\right)=0.
\end{equation}
The preceding equation determines $m$ as a function of $x$ and $j$.
\end{proof}


\begin{proposition}
  Let $m(x,j)$ be determined by {\color{red}3.21}. If $j>0$, then, \eqref{cost} becomes
\begin{equation}\label{costjpos}
c_{01}(j)=\int_0^1 D_vL(x,\frac{j}{m(x,j)},m(x,j)).
\end{equation}
Similarly, if $j<0$, then, \eqref{cost10} becomes
\begin{equation}\label{costjpos}
c_{10}(j)=-\int_0^1 D_vL(x,\frac{j}{m(x,j)},m(x,j)).
\end{equation}
\end{proposition}
\begin{proof}
\end{proof}

% \paragraph{The cost for $j>0$: }
% When $j>0$, we know a bit more.
% From optimal control theory
% \begin{equation}\label{v1}
% v^*(x,j)=-D_pH(x,u_x(x,j),m(x,j)),
% \end{equation}
% and from the second equation in \eqref{mfgsys} \begin{equation}\label{v2}
% v^*(x,j)=\frac{j}{m(x,j)}.
% \end{equation}


\paragraph{ Monotonicity of the costs}
Now, we examine the monotonicity properties of the costs.


For general MFGs of the form \eqref{MFGgeneral}, 
under the condition that
\begin{gather}\label{matrix}
    \begin{bmatrix}
    -\frac{2}{m}D_mH & D^2_{pm}H \\
    D^2_{pm}H & 2D^2_{pp}H
    \end{bmatrix}\geq 0
    \end{gather}
the uniqueness of solution in a number of cases was proved in \cite{cursolions} and \cite{porretta}.


Now, we begin our analysis by considering $c_{01}$ when $j>0$.

\begin{proposition}
    see proof!
\end{proposition}
\begin{proof}Assuming $j>0$, and differentiating \eqref{mfgsys} with respect to $j$, we get
\begin{equation}\label{dj}
\begin{cases}
\begin{aligned}
 -D_pH(x,-c_{01},m) \frac{\partial c_{01}}{\partial j}+D_mH(x,-c_{01},m) \frac{\partial m}{\partial j}&=0, \\
 mD^2_{pp}H(x,-c_{01},m)\frac{\partial c_{01}}{\partial j} -\left(D_pH(x,-c_{01},m)+ 
mD^2_{pm}H(x,-c_{01},m\right)\frac{\partial m}{\partial j}&=1,
\end{aligned}
\end{cases}
\end{equation}
where $c_{01}=c_{01}(x,j)$ and $m=m(x,j)$.
From the first equation in \eqref{dj}, we have
\begin{equation}
\frac{\partial c_{01}}{\partial j}=- \frac{mD_mH(x,-c_{01},m)}{j}\frac{\partial m}{\partial j}.
\end{equation}
Thus, if $D_mH(x,-c_{01},m) \leq 0$, then $m$ and $c_{01}$ have the same monotonicity with respect to $j$ and opposite otherwise.

The solution of \eqref{dj} is
\begin{gather}\label{djsol}
\begin{bmatrix}
\frac{\partial c_{01}}{\partial j} \\
\frac{\partial m}{\partial j}
\end{bmatrix}
=
\frac{1}{(D_pH)^2+mD_pHD_{pm}^2H-D_mHD_{pp}^2Hm}
\begin{bmatrix}
-D_mH \\
-D_pH
\end{bmatrix}.
\end{gather}

% \begin{result}
% \end{result}
Notice that the determinant of the matrix in \eqref{matrix} is
$$
A=-\frac{4}{m}D_mHD^2_{pp}H-(D^2_{pm}H)^2 \geq 0.
$$
Using this and by Cauchy's inequality, we get that the denominator in \eqref{djsol}
\begin{equation*}
\begin{aligned}
&(D_pH)^2+mD_pHD_{pm}^2H-D_mHD_{pp}^2Hm \\
& \geq (D_pH)^2-(D_pH)^2- \frac{1}{4}m^2(D^2_{pm}H)^2-D_mHD^2_{pp}Hm \\
& = \frac{Am^2}{4} \geq 0.
\end{aligned}
\end{equation*}
Condition \eqref{matrix} implies
$$
\frac{\partial c_{01}}{\partial j} \geq 0.
$$
\end{proof}
However, {\color{red}3.30} is not necessary for monotonicity of the cost, as
we show in the next example for separable Hamiltonians.
%{\color{red}
%Need to think of $c_{01}$ vs ${c_{10}}$ here.
%}
\begin{example}
Suppose $H$ is separable, i.e.
\[
D^2_{pm}H=0\ \text{and} \ D_mH=-g^{\prime}(m).
\]
From \eqref{djsol}, we get
\begin{equation}\label{dc1}
\frac{\partial c_{01}}{\partial j}=\frac{g^{\prime}(m)}{(D_pH)^2+D_{pp}Hmg^{\prime}(m)}.
\end{equation}
If $g^{\prime}(m) >0$ then $\frac{\partial c_{01}}{\partial j} \geq 0$.
If $g^{\prime}(m) <0$, the analysis is more delicate.

Let $\gamma>1$. Consider the case where
\[
H(p,m)=\frac{|p|^\gamma}{\gamma}-g(m).
\]
Then, we have
\begin{equation*}
\begin{aligned}
& D_pH(p,m) = p|p|^{\gamma -2}, \\
& D_pH(p,m)^2=|p|^{2\gamma -2}\implies (D_pH(-c_{01},m))^2=(\gamma g(m))^{2-\frac{2}{\gamma}}, \\
& D^2_{pp}H(p,m)= (\gamma-1)|p|^{\gamma -2}\implies D^2_{pp}H(-c_{01},m)=
(\gamma-1)(\gamma g(m))^{1-\frac{2}{\gamma}}.
\end{aligned}
\end{equation*}
%\begin{equation*}
%\begin{aligned}
%& D_pH = p|p|^{\gamma -2}, \\
%& (D_pH)^2=p^2|p|^{2(\gamma -2)}=(\gamma g(m))^{\frac{2}{\gamma}}(\gamma g(m))^{2-\frac{4}{\gamma}}, \\
%& D^2_{pp}H= |p|^{\gamma -2}+(\gamma-2)p^2|p|^{\gamma -4}=
%(\gamma g(m))^{1-\frac{2}{\gamma}}+(\gamma-2)(\gamma g(m))^{\frac{2}{\gamma}}(\gamma g(m))^{1-\frac{4}{\gamma}}.
%\end{aligned}
%\end{equation*}
Substituting in \eqref{dc1}, we get
\begin{equation}
\frac{\partial c_{01}}{\partial j}=\frac{g^{\prime}(m)}{(\gamma g(m))^{2-\frac{2}{\gamma}}+(\gamma-1)(\gamma g(m))^{1-\frac{2}{\gamma}}mg^{\prime}(m)}.
\end{equation}
Thus, to get $\frac{\partial c_{01}}{\partial j} \geq 0$ when $g^{\prime}(m) <0$, we need
\begin{equation}\label{cond}
\gamma g(m) +(\gamma -1)m g^{\prime}(m) \leq 0.
\end{equation}
A case where the prior inequality holds is the following.
Consider
$$g(m)=m^{-\beta}, \ \beta>0.$$
Then \eqref{cond} becomes
$$\gamma-(\gamma-1)\beta \leq 0.$$
Hence, for
$\beta \geq \frac{\gamma}{\gamma-1}, $
we have $\frac{\partial c_{01}}{\partial j} \geq 0$.
\end{example}

Now, we study the monotonicity of $c_{01}$ for $j \leq 0$.
\begin{proposition}
\end{proposition}
\begin{proof}
    
    We write \eqref{DvL} as follows
    $$
    v(x,j)D_vL(x,v(x,j),m(x,j))-L(x,v(x,j),m(x,j))=0.
    $$
    Then, we differentiate with respect to $j$, to get
    \begin{equation}\label{DvvL}
        \begin{aligned}
            & v(x,j)D^2_{vv}L(x,v(x,j),m(x,j))\frac{\partial v(x,j)}{\partial j}
            +v(x,j)D^2_{vm}L(x,v(x,j),m(x,j))\frac{\partial m(x,j)}{\partial j} \\
            & -D_mL(x,v(x,j),m(x,j))\frac{\partial m(x,j)}{\partial j}=0.
        \end{aligned}
    \end{equation}
    Also, differentiating \eqref{cost} with respect to $j$, we get
    \begin{equation*}
        \begin{aligned}
            & \frac{\partial c_{01}(j)}{\partial j} = \int_0^1
            D^2_{vv}L(x,v(x,j),m(x,j))\frac{\partial v(x,j)}{\partial j} \\
            & +D^2_{vm}L(x,v(x,j),m(x,j))\frac{\partial m(x,j)}{\partial j} dx.
        \end{aligned}
    \end{equation*}
    Substituting $D^2_{vv}L(x,v(x,j),m(x,j))$ from \eqref{DvvL}, we get
    $$
    \frac{\partial c_{01}(j)}{\partial j} = \int_0^1 {\frac{1}{v} D_mL(x,v(x,j),m(x,j))\frac{\partial m(x,j)}{\partial j}} dx \geq 0.
    $$
    Thus the cost is monotone.
\end{proof}
    
\paragraph{Reversibility of the cost}
Now, we study the reversibility of the cost and its dependence to the reversibility of the Hamiltonian.
\begin{proposition}
If the Hamiltonian is reversible $(H(-p)=H(p))$, then the cost is reversible, that is, $c_{01}(j)=c_{10}(j), \ \forall j \in \mathbb{R}$.
%This means that the cost for traveling along an edge from right to left is the same as the cost for traveling from left to right along the same edge.
\end{proposition}
\begin{proof}
Since $H$ is reversible, $L$ is also reversible i.e.
$$
L(-v)=L(v).
$$
$m$ is given by solving \eqref{m}.
For $j>0$, traveling from $0$ to $1$, the optimal velocity is $v=\frac{j}{m}$, which solves the necessary optimality condition \eqref{L/v}.
For same $j$ and $m$, we look at the optimal trajectory connecting $1$ to $0$.
We claim that the velocity $-v$ is optimal.
This is true because $-v$ also solves \eqref{L/v}.
Then by \eqref{cost}, we have
$$c_{01}(j)=c_{10}(j).$$
Thus, the cost is reversible.
\end{proof}
%reversibility implies also,
%$$m(x,j)=m(x,-j).$$
%$$c_{01}(j)=c_{01}(-j).$$
%Perhaps, for some cases we have $m(x,j)=m(x,-j).$, without reversibility.
\begin{example}[Reversible Hamiltonian]
Suppose the Hamiltonian is
$$
H(x,p,m)=\frac{p^2}{2}-m.
$$
Then, the Lagrangian is
$$
L(x,v,m)=\frac{v^2}{2}+m,
$$
and the MFG system is
\begin{equation*}
\begin{cases}
\frac{u_x^2}{2}=m,\\
(-mu_x)_x=0.
\end{cases}
\end{equation*}
$m$ is obtained by substituting $u_x=-\frac{j}{m}$ in the HJ equation
$$
\frac{1}{2} \left( -\frac{j}{m} \right) ^2=m,
$$
then
$$
m=\left( \frac{j^2}{2} \right) ^{1/3}.
$$
On the other hand, \eqref{DvL} implies
$$
v=(2m)^{1/2}.
$$
Hence, substituting the formula for $m$ in the previous identity, we get
$$
v=\left( 2 \left( \frac{j^2}{2} \right) ^{1/3} \right) ^{1/2}.
$$
Then, by \eqref{cost} the cost is
$$
c_{01}(j)=\int_0^1 2^{1/3} |j|^{1/3} dx = 2^{1/3}|j|^{1/3}.
$$
This cost is actually independent of the sign of $j$ because the Hamiltonian is reversible.
We can see this using \eqref{costjpos}, where we get the same cost
$$
c_{01}(j)=\int_0^1 \frac{j}{m} = \frac{j}{(j^2/2)^{1/3}}=(2j)^{1/3}.
$$
\end{example}
\begin{example}[Non-reversible Hamiltonian]
The cost may be assymmetric, i.e.
$c_{01}(j)$ and $c_{10}(j)$ may be different.
Suppose the Hamiltonian is
\[
H(x,p,m) = \frac{p^4}{4}- \beta p -m.
\]

The $-\beta p$ term indicates that agents have a preference to move to the right with velocity $\beta$.
The corresponding Lagrangian is $L(v,m) = \frac{3}{4}(v-\beta)^{4/3}+m$.

Solving the corresponding MFG system for $m$ as a function of $j$, with $\beta=2$, we obtain {\color{red}check mathematica notebook costplots.nb in section critical congestion, non-quadratic}
\[
m(j)= 6^2+4j(2m-j)+2j(2m-j)^3+(2m-j)^4+(2m-j)^6,
\]
i.e.
$2 m(j)-j$ is
the second root (from $-\infty$ to $\infty$) of the following polynomial in $x$:
\[
j^2+4j x+2j x^3+ x^4+x^6
\]
elevated to the power 3.

It is easy to see that the polynomial changes as the sign of $j$ changes.
\end{example}

\subsubsection{Relevance and interpretation of the results}
Crowd aversion is Lions monotonicity condition, i.e.
both $c$ and $m$ increase with $j$.
It is possible, however, to have a crowd seeking behavior, i.e.
$g$ decreasing with $c$ increasing in $j$ but in this case $m$ decreases with $j$.

This is actually something that happens in uncongested highways.
As speed increases, cars increase their distances, hence density decreases.
Let us look at the velocity in \eqref{v2}, this is the optimal velocity at which the agents move.
Now, we answer the question: what happens to the velocity as a function of $j$ ?

Differentiating \eqref{v2}, with respect to $j$, we get
\begin{equation*}
\frac{\partial}{\partial j}\left[v(x,j)\right]=
\frac{1}{m} - \frac{j}{m^2} \frac{\partial m}{\partial j}.
\end{equation*}
From \eqref{djsol} and using \eqref{v1}, we have
$$
\frac{\partial m(x,j)}{\partial j}= \frac{-D_pH}{M} =\frac{j}{m M},
$$
where $M=(D_pH)^2+mD_pHD_{pm}^2H-D_{pp}^2HD_mHm$.
Hence
$$
\frac{\partial}{\partial j}\left[v(x,j)\right]=
\frac{1}{m}\left[ 1-\frac{j^2}{m^2}\frac{1}{M} \right]=
-\frac{1}{m} \frac{mvD^2_{pm}H+D^2_{pp}HD_mHm}{M}.
$$
In the separable case, we have
$$
\frac{\partial}{\partial j}\left[v(x,j)\right]=-\frac{1}{m}\frac{D^2_{pp}Hg^{\prime}(m)m}{M}.
$$
So, if reverse Lions condition holds
$$
\frac{\partial}{\partial j}\left[v(x,j)\right] \geq 0.
$$
Another quantity of interest is
$$\frac{\partial m(x,j)}{\partial v(x,j)} \geq 0,$$
which corresponds to uncongested model.
In the separable case, we have
$$
\frac{\partial m(x,j)}{\partial v(x,j)}= -\frac{v}{D^2_{pp}Hg^{\prime}(m)m}.
$$
If $g^{\prime}(m)$ increasing, $m$ decreases with $v$.
Whereas if $g^{\prime}(m)$ decreasing, $m$ increases with $v$.
This is independent on $m$.
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mean-field game model on a network}\label{MFG model}

Now, we examine the MFG formulation on networks.
Our MFG model consists of the network, the data given on the network, the variables and the equations connecting these variables.

\subsubsection{The network and the data}
In the MFG model, we are given the following
\begin{itemize}
\item A finite \textbf{undirected} network, $\Gamma=(E,V)$, where
$E = \{e_k : k \in \{1,2,\dots,n\} \}$ is the set of edges
and $V=\{v_i : i \in \{1,2,\dots, m\} \}$ is the set of vertices.
We write $e_k=(v_r,v_i)$.
\item Agents enter the network through {\em entrance vertices} and exit it through {\em exit vertices}.
To every entrance vertex, $v_i$, we associate an auxiliary edge, $e_k=(v_r,v_i)$, called the {\em entrance edge}.
Similarly, to every exit vertex, $v_i$, we associate an auxiliary edge, $e_l=(v_i,v_s)$, called {\em exit edge}.

Sometimes, the original edges of the network will be called basic edges, to distinguish between them and the auxiliary edges.
\item A flow of agents, the entry current $\iota >0$, is prescribed at entrance vertices.
The entry currents in the other vertices are zero.
This information is encoded in the $m$-dimensional vector $B$.
At the exit vertices, the exit cost $\bar{u}$ is given.
\end{itemize}

\subsubsection{The variables and the costs}
On the network $\Gamma$, we define the following variables
\begin{enumerate}
\item \textbf{Edge currents:} The \emph{current} $j_k$ in the edge $e_k=(v_r,v_i)$ is decomposed in positive and negative parts, $j_k= j_k^i-j_k^r$ such that
\begin{equation}\label{js}
j_k^i \cdot j^r_k=0, \ \ j_k^i, j^r_k \geq 0.
\end{equation}
where $j^i_k$ is the current going to the vertex $v_i$ and $j^r_k $ is the current going to the vertex $v_r$.
This means that all agents in an edge move in the same direction.
\item \textbf{Transition currents:}
The \emph {transition current} from $e_k$ to $e_l$ through a common vertex is denoted by $j_{kl}$.
The transition currents also satisfy the complementary condition
\begin{equation}\label{jts}
j_{kl} \cdot j_{lk}=0, \ \ j_{kl}, j_{lk} \geq 0.
\end{equation}
\item \textbf{Value functions:}
The \emph{value function} in the edge $e_k=(v_r,v_i)$ at the vertex $v_i$ is denoted by $u_k^i$.
\end{enumerate}
On $\Gamma$, we also have the following costs
\begin{itemize}
\item \textbf{Travel costs:}
In the edge $e_k=(v_r,v_i)$, the cost of moving from $v_r$ to $v_i$ is $c_{ri}(j_k)$, and the cost of moving from $v_i$ to $v_r$ is $c_{ir}(j_k)$.
In our MFG, the cost in the edge depends only on the current in this edge.
\item \textbf{Switching costs:}
For moving from $e_k$ to $e_l$ through a common vertex, agents pay a \emph{switching cost}, $\psi_{kl}$.
Often, we may require $\psi_{kl} \geq 0$.
The switching cost from an entry edge to a basic edge is $0$, and from a basic edge to an entry edge is $\infty$.
Similarly, the switching cost from an exit edge to a basic edge is $\infty$, and from a basic edge to an exit edge is $0$.
\begin{remark} This avoids entry through exits and exit through entrances.
\end{remark}
For any vertex, $v_i$, that has more than two incident edges, we require the following triangle-type inequality in the switching costs,
\[
\psi_{kl} \leq \psi_{km}+ \psi_{ml}.
\]
\end{itemize}

\subsubsection{The equations}
The variables are related to each other through the following equations and inequalities
\paragraph*{\textbf{Optimality conditions at the vertices}}
In the process of minimizing their travel cost, agents choose the least expensive path.
They decide to switch from $e_k$ to $e_l$ through the common vertex $v_i$, if
\begin{equation}\label{optcond}
u^i_k\leq \min\limits_{l \in \mathcal{K}} \big\{ u_l^i + \psi_{kl} \big\}.
\end{equation}
\paragraph*{\textbf{Complementarity conditions at the vertices}}
If the transition current $j_{kl}$ is not zero, then the agents are moving from $e_k$ to $e_l$ through $v_i$.
This implies that $u_k^i+ \psi_{kl}=u_l^i$.
So, we have the following,
\begin{equation}\label{ujcomp}
j_{kl} \cdot (u^i_l- u^i_k +\psi_{kl})=0, \ \forall i, k, l.
\end{equation}
\paragraph*{\textbf{Optimality conditions in the edges}}
In the edge $e_k=(v_r,v_i)$, for any $j_k$ we have
\begin{equation}\label{optcond2}
\begin{cases}
u^r_k \leq c_{ri}(j_k) + u_k^i, \\
u^i_k \leq c_{ir}(j_k) + u^r_k.
\end{cases}
\end{equation}
For $j_k>0$, \eqref{optcond2} becomes
$$
u^r_k = c_{ri}(j_k^i) + u_k^i.
$$
For $j_k<0$, \eqref{optcond2} becomes
$$
u_k^i= c_{ir}(-j_k^r) + u^r_k.
$$

The costs $c_{ri}(j_k^i)$ and $c_{ir}(-j_k^r)$ may not be the same, unless the system is reversible.
\paragraph*{\textbf{Complementarity conditions in the edges}}
In the edge $e_k=(v_r,v_i)$, we have the complementary conditions
\begin{equation}\label{compedge}
\begin{cases}
j_k^i \cdot (u_k^r-u_k^i-c_{ri}(j_k))=0, \\
j_k^r \cdot (u_k^i-u_k^r-c_{ir}(j_k)=0.
\end{cases}
\end{equation}
%which can be written in the following way
%$$
%j_k^i >0 \Rightarrow \ u_k^r-u_k^i-c_{ri}(j_k)=0,
%$$
%or
%$$
%j_k^i =0 \Rightarrow \ u_k^r-u_k^i-c_{ri}(j_k) \geq 0.
%$$
\paragraph*{\textbf{Kirchhoff's law and the balance equations}}
Consider the edge $e_k=(v_r,v_i)$, and let all the incident edges to $e_k$ at $v_r$ be denoted by $e_l=(v_s,v_r)$ ($l$ and $s$ are not fixed).
The Kirchhoff's law at $v_r$ is
\begin{equation}\label{Kirch}
j_k=\sum_l j_l,
\end{equation}
which can be written using the current decomposition
$$
j_k^i-j_k^r= \sum_l (j_l^r-j_l^s).
$$
In terms of the transition currents, the current $j_k^r$ is equal to the sum of the transition currents from $e_k$ to all the other incident edges at $v_r$, this models a splitting of the current.
\begin{equation}\label{balance1}
\sum_l j_{kl}=j^k_r.
\end{equation}
We have a similar equation for the gathering of the transition currents, the current $j_k^i$ is the sum of the transition currents from all the incident edges at $v_r$ to $e_k$.
\begin{equation}\label{balance2}
\sum_l j_{lk}= j^i_k.
\end{equation}

If $j_{kl} > 0 $, then $u$ has Dirichlet boundary condition at the right for the HJ equation.
The gathering equation determines the boundary condition at the left for the transport equation.
\paragraph*{\textbf{Entry edge equations}}
In every entry edge $e_k=(v_r,v_i)$, given the entering current $\iota$ at the entrance vertex $v_i$, we have
\begin{equation}\label{incondj}
\begin{cases}
j^i_k=\iota.\\
j^r_k=0.
\end{cases}
\end{equation}
In $e_k$, we also, have
\begin{equation}\label{incondu}
u^r_k=u^i_k.
\end{equation}

\paragraph*{\textbf{Exit edge equations}}
In every exit edge $e_l=(v_i,v_s)$, given the exit cost $\bar{u}$ at the exit vertex $v_i$, we have
\begin{equation}\label{outcondu}
u^s_l = u^i_l = \bar{u}.
\end{equation}
In $e_l$, we also have
\begin{equation}\label{outcondj}
j^i_l=0.
\end{equation}

%\paragraph*{\textbf{Basic edge equation}}
%In the each basic edge, we have
%\begin{equation}\label{edgeeq}
%j\int_0^1m^{\alpha-1}dx=u(0)-u(1).
%\end{equation}
%or
%$$
%(j_k^i-j_k^r) \int_0^1m_k^{\alpha-1}dx=u_k^r-u_k^i.
%$$

%$u(0)-u(1)=c(j_k^i-j_k^r)\sgn(j_k^i-j_k^r).$


Now, we present a simple example to illustrate this framework.
\begin{IMG}
{"1edge", Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 1]]},
VertexLabels -> {1 -> Subscript["v", 1], 2 -> Subscript["v", 2]}, GraphLayout -> "RadialDrawing"](*\]*)}	
\end{IMG}
\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge.pdf}
\caption{Simple network with one edge.}
\end{figure}
\begin{IMG}
{"1edge2", Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 0]],
Labeled[2 \[DirectedEdge] 3, Subscript["e", 1]],
Labeled[3 \[DirectedEdge] 4, Subscript["e", 2]]},
VertexLabels -> {1 -> Subscript["v",0], 2 -> Subscript["v", 1],
3 -> Subscript["v", 2],4 -> Subscript["v", 3]},
EdgeStyle -> {1 \[DirectedEdge] 2 -> Dashed,
3 \[DirectedEdge] 4 -> Dashed},
GraphLayout -> "RadialDrawing"](*\]\]\]\]\]*)}	
\end{IMG}
\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge2.pdf}
\caption{One edge network with entrance and exit edges.}
\label{1edgegrapgh}
\end{figure}
\begin{example}\label{1edge}
Consider a network of one edge as in Fig \ref{1edgegrapgh}, $e_1=(v_1,v_2)$.
Given an entry current $\iota >0$ at the entrance vertex $v_1$, and the exit cost $\bar{u}$ at the exit vertex $v_2$
Assuming $e_{0}=(v_0,v_1)$ is the entrance edge and $e_2=(v_2,v_3)$ is the exit edge.
For simplicity we set all the switching costs to zero.
We consider the MFG \eqref{mfgs} and write the corresponding equations in the critical congestion case, i.e.
$\alpha=1$.
In the critical congestion case, from the second equation in \eqref{current mfg}, the cost is $j$.
\begin{itemize}
\item
\eqref{js} gives
\begin{equation*}
\begin{cases}
j_0^1 \cdot j_0^0 =0, \ j_0^1,j_0^0 \geq 0, \\
j_1^2 \cdot j_1^1 =0, \ j_1^2,j_1^1 \geq 0, \\
j_2^3 \cdot j_2^2 =0, \ j_2^3,j_2^2 \geq 0.
\end{cases}
\end{equation*}
\item
\eqref{jts} gives
\begin{equation*}
\begin{cases}
j_{01} \cdot j_{10} =0, \ j_{01},j_{10} \geq 0, \\
j_{12} \cdot j_{21} =0, \ j_{12},j_{21} \geq 0.
\end{cases}
\end{equation*}
\item
\eqref{optcond} gives
\begin{equation*}
\begin{cases}
u_0^1 \leq u_1^1, \ u_1^1 \leq u_0^1, \\
u_1^2 \leq u_2^2, \ u_2^2 \leq u_1^2.
\end{cases}
\end{equation*}

Which implies $u_0^1 = u_1^1$ and $u_1^2= u_2^2$.
\item
\eqref{ujcomp} gives
\begin{equation*}
\begin{cases}
j_{10} \cdot (u_0^1 - u_1^1)=0, \ j_{01} \cdot (u_1^1 - u_0^1)=0, \\
j_{21} \cdot (u_1^2 - u_2^2)=0, \ j_{12} \cdot (u_2^2 - u_1^2)=0.
\end{cases}
\end{equation*}
\item
\eqref{optcond2} gives
\begin{equation}
\begin{cases}
u_0^0 \leq j_0 + u_0^1, \
u_0^1 \leq j_0 + u_0^0, \\
u_1^2 \leq j_1 + u_1^1, \
u_1^1 \leq j_1 + u_1^2, \\
u_2^2 \leq j_2 + u_2^3, \
u_2^3 \leq j_2 + u_2^2.
\end{cases}
\end{equation}
\item
\eqref{compedge} gives
\begin{equation}
\begin{cases}
j_0^1 \cdot ( u_0^0 - u_0^1 - j_0 )=0, \
j_0^0 \cdot ( u_0^1 - u_0^0 - j_0 )=0, \\
j_1^1 \cdot ( u_1^2 - u_1^1 - j_1 )=0, \
j_1^2 \cdot ( u_1^1 - u_1^2 - j_1 )=0, \\
j_2^3 \cdot ( u_2^2 - u_2^3 - j_2 )=0, \
j_2^2 \cdot ( u_2^3 - u_2^2 - j_2 )=0.
\end{cases}
\end{equation}

\item
\eqref{balance1} and \eqref{balance2} give
\begin{equation*}
\begin{cases}
j_0^1=j_{01}, \ j_0^0=j_{10}, \\
j_1^2=j_{12}, \ j_1^1=j_{10}, \\
j_1^2=j_{01}, \ j_1^1=j_{21}, \\
j_2^3=j_{12}, \ j_2^2=j_{21}.
\end{cases}
\end{equation*}
\item \eqref{incondj} and \eqref{incondu} give
\begin{equation*}
\begin{cases}
j_0^1= \iota, \ j_0^0=0, \\
u_0^0= u_0^1.
\end{cases}
\end{equation*}
\item \eqref{outcondj} and \eqref{outcondu} give
\begin{equation*}
\begin{cases}
u_2^2 =u_2^3= \bar{u},\\
j_2^2 = 0.
\end{cases}
\end{equation*}
%\item The last equation in \eqref{current mfg} gives the edge equation
%$$
%u_1^1-u_1^2= j_1^2-j_1^1.
%$$
\end{itemize}
\end{example}
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsection{Reformulation of mean-field game as Wardrop model}\label{MFGtoW}

Now, we reformulate the MFG model in Section \ref{MFG model} to a Wardrop equilibrium model as the one described in Section \ref{Wmodel}.
We then, show that given the MFG solution, we have a Wardrop equilibrium.
For this, we identify the network, the currents and the costs in the Wardrop model.

In Wardrop, the network $\tilde{\Gamma}$ is directed but in MFG the network $\Gamma$ is undirected.
In $\Gamma$, we double the undirected edges so that every edge is directed with the same vertices, and we blow-up the connecting vertices into a set of pairs of auxiliary edges called \emph{transition edges}.
Now, we have an extended directed network $\bar{\Gamma}$ for the MFG model.
In this new network, we have the following
\begin{itemize}

\item Every current $j_k^i$ or transition current $j_{kl}$, corresponds to a positive current in a directed edge of $\bar{\Gamma}$.
The transition currents are edge currents in the transition edges.

\item We write Kirchhoff's law as follows
$$
j_k^i+ \sum_l j_l^s = j_k^r +\sum_l j_l^r.
$$

\item We consider the matrix $K$ that represents Kirchhoff's law, %equations \eqref{balance1}, \eqref{balance2},
\eqref{incondj} and \eqref{outcondj}, as $K\bm{\jmath}=B$.
Each column in $K$ corresponds to a current and hence to an edge.
Each row corresponds to a vertex.
Some currents in the network will appear in two rows of $K$.
These two rows give the two vertices of the corresponding edge.
Some appear only once.
These are the exit vertices and we simply add a vertex which is a sink and hence there is no need for a further balance equation there.


\item In the undirected edge $e_k=(v_r,v_i)$, based on the discussion in Section \ref{costsection}, we have two costs $c_{ri}(j_k)$ and $c_{ir}(j_k)$.
We double $e_k$ to make it directed, so we have the edge $e_{\tilde{k}}=(v_i,v_r)$.
In this case, we have the current $j_k^i$ in $e_k$, and the current $j_{\tilde{k}}^r$ in $e_{\tilde{k}}$.
The cost for traveling from $v_r$ to $v_i$ in $e_k$ is $\bar{c}_{ri}(\bm{j_k})=c_{ri}(j_k^i-j_{\tilde{k}}^r)$, where $\bm{j_k}=(j_k^i,j_{\tilde{k}}^r)$,
and the cost for traveling from $v_i$ to $v_r$ is $\bar{c}_{ir}(\bm{j_k})=c_{ir}(j_{\tilde{k}}^r-j_k^i)$.


% where $\bm{j_{\tilde{k}}}=(j_{\tilde{k}}^r,j_k^i)$.
%$\bar{c}_{ir}(j_{\tilde{k}}^r-j_k^i)$.

%If we double $e_k$ to make it direct, we get the edge $e_{\tilde{k}}=(v_{\tilde{r}},v_{\tilde{i}})$.
%In this case, we have the current $j_k^i$ in $e_k$, and the current $j_{\tilde{k}}^{\tilde{r}}$ in $e_{\tilde{k}}$.
%The cost for traveling from $r$ to $i$ in $e_k$ is denoted by $\hat{c}_{ri}(j_k^i-j_{\tilde{k}}^{\tilde{r}})$, and the cost for traveling from $\tilde{i}$ to $\tilde{r}$ is denoted by $\hat{c}_{\tilde{i}\tilde{r}}(j_{\tilde{k}}^{\tilde{r}}-j_k^i)$.

%These two costs are related to each other as follows
%\begin{equation}\label{extended cost}
%\hat{c}(\hat{j})=c_{ri}(\hat{j})-c_{\tilde{i}\tilde{r}}(\hat{j}),
%\end{equation}
%where $\hat{j}=j_k^i-j_{\tilde{k}}^{\tilde{r}}$.

%$$\hat{c}=c_{01}(j)-c_{10}(j).$$

%\begin{equation*}
%c_k(j_k^i,j_k^r)=
%\begin{cases}
%+\infty \ \text{if} \ j_k^i \neq 0 \ \text{and} \ j_k^r \neq 0, \\
%c(j_k^i) \ \text{otherwise}.
%\end{cases}
%\end{equation*}


\item The switching costs $\psi_{kl}$ turn into constant travel costs in the transition edges.

\item To make the exit cost $\bar{u}$ at the exit vertex $v_r$ zero, we add an auxiliary edge $e_k=(v_r,v_i)$ incident to $v_r$ such that the exit cost at $v_i$ is zero and in the auxiliary edge the cost is $c(j_k^i)=\bar{u}$.




\end{itemize}


Now, we present the main theorem that connects the MFGs with the Wardrop model.
\begin{theorem}
If $\bm{{\jmath}^*}$ is a solution to the MFG system, then it is also a solution to the new Wardrop model with the new costs $\bar{c}_{ri}(\bm{j_k})$ and $\bar{c}_{ir}(\bm{j_k})$.
\end{theorem}
\begin{proof}
For admissible $\bm{{\jmath}^*}$ and $\bm{\jmath}$, we have
$$
K \bm{{\jmath}^*}=B \ \text{and} \ K \bm{\jmath}=B.
$$
Subtracting the two equations, we get
$$
K(\bm{{\jmath}^*} - \bm{\jmath})=0.
$$
Multiplying by $\bm{u^{T}}$, where $\bm{u^{T}}$ is the vector of the value functions
$$
\bm{u^{T}}K(\bm{{\jmath}^*}-\bm{\jmath})=0,
$$
each current appears twice, one for each of its vertices but with different signs.
The previous computation yield
$$
\sum (u_k^r-u_k^i)(j^{i*}_k-j_k^i)=0.
$$
Now, we have two cases
$$
j^{i*}_k > 0 \Rightarrow u_k^r-u_k^i=\bar{c}_{ri}(\bm{j_k}^*),
$$
or
$$
j^{i*}_k =0 \Rightarrow u_k^r-u_k^i \geq \bar{c}_{ri}(\bm{j_k}^*).
$$
This implies
$$
\langle \bar{c}_{ri}(\bm{{\jmath}^*}), \bm{{\jmath}^*}-\bm{\jmath} \rangle \leq 0.
$$
Similarly, we get
$$
\langle \bar{c}_{ir}(\bm{{\jmath}^*}), \bm{{\jmath}^*}-\bm{\jmath} \rangle \leq 0,
$$
which is a Wardrop equilibrium.
\end{proof}

Next, we study the monotonicity of the cost.
\begin{proposition}
If the cost is reversible and increasing in the MFG, then the Wardrop equilibrium is unique.
\end{proposition}
\begin{proof}
For an edge $e_k=(v_r,v_i)$, let $\bar{c}_{ri}(\bm{j_k})=c_{ri}(j_k^i-j_{\tilde{k}}^r)=c_{ri}(j_k)$ be the cost in the new Wardrop, where $c_{ri}$ is the cost in the MFG,
$\bm{j_k}=(j_k^i,j_{\tilde{k}}^r)$.
% and $j_k=j_k^i-j_{\tilde{k}}^r$.
Similarly, let $\bar{c}_{ir}(\bm{j_k})=c_{ir}(j_k^i-j_{\tilde{k}}^r)=c_{ir}(-j_k)$.
For the Wardrop monotonicity, we need monotonicity over all edges i.e.
$$
\sum_k (c_k({\bm{\tilde{\jmath}}})-c_k({\bm{\hat{\jmath}}}),
{\bm{\tilde{\jmath}}}-{\bm{\hat{\jmath}}}) \geq 0,
$$
which can be written for each edge
$$
\sum_k (\bar{c}_{ri}({\bm{\tilde{\jmath}}})- \bar{c}_{ri}({\bm{\hat{\jmath}}}),
{\bm{\tilde{\jmath}}}-\bm{\hat{\jmath}} ) +
(\bar{c}_{ir}({\bm{\tilde{\jmath}}})- \bar{c}_{ir}({\bm{\hat{\jmath}}}),
{\bm{\tilde{\jmath}}}-\bm{\hat{\jmath}}) \geq 0.
$$
%By the monotonicity in the MFG, (i.e.
%$c_{ri}$ and $c_{ir}$ are monotone), we get
Or
$$
\sum_k (c_{ri}({\tilde{\jmath}}_k)- c_{ri}({\hat{\jmath}}_k),
{\tilde{\jmath}}_k^i - {\hat{\jmath}}_k^i ) +
(c_{ir}(-{\tilde{\jmath}}_k)- c_{ir}(-{\hat{\jmath}}_k),
{\tilde{\jmath}}_k^r - {\hat{\jmath}}_k^r) \geq 0.
$$
If the cost is reversible (i.e.
$c_{ri}(j)=c_{ir}(j)=c(j)$), we get
\begin{equation}\label{revcost}
\sum_k (c({\tilde{\jmath}}_k)- c({\hat{\jmath}}_k),
{\tilde{\jmath}}_k^i - {\hat{\jmath}}_k^i ) +
(c(-{\tilde{\jmath}}_k)- c(-{\hat{\jmath}}_k),
{\tilde{\jmath}}_k^r - {\hat{\jmath}}_k^r) \geq 0.
\end{equation}
For Wardrop equilibrium, we verify four cases, these cases are as follows
\begin{enumerate}
\item Case 1: ${\tilde{\jmath}}_k^r={\hat{\jmath}}_k^r=0$.
In this case, \eqref{revcost} becomes
$$
\sum_k (c({\tilde{\jmath}}_k^i)-c({\hat{\jmath}}_k^i),{\tilde{\jmath}}_k^i-{\hat{\jmath}}_k^i) \geq 0.
$$
This is true, since the cost $c(j)$ is increasing for $j>0$.
Note that the inequality is strict if $c(j)$ is strictly increasing and ${\tilde{\jmath}}_k^i \neq {\hat{\jmath}}_k^i$.
\item Case 2: ${\tilde{\jmath}}_k^i={\hat{\jmath}}_k^i=0$.
In this case, for symmetric $c$, \eqref{revcost} becomes
$$
\sum_k (c(-{\tilde{\jmath}}_k^r)-c(-{\hat{\jmath}}_k^r),{\tilde{\jmath}}_k^r-{\hat{\jmath}}_k^r) \geq 0.
$$
This is true, since the cost $c(j)$ is increasing for $j>0$.
\item Case 3: ${\tilde{\jmath}}_k^i={\hat{\jmath}}_k^r=0$.
In this case, for symmetric $c$, \eqref{revcost} becomes
$$
\sum_k (c({\tilde{\jmath}}_k^r)-c({\hat{\jmath}}_k^i),{\tilde{\jmath}}_k^r-{\hat{\jmath}}_k^i) \geq 0.
$$
This is true, for symmetric $c$, since the cost $c(j)$ is increasing for $j>0$.
\item Case 4: ${\tilde{\jmath}}_k^r={\hat{\jmath}}_k^i=0$.
In this case, \eqref{revcost} becomes
$$
\sum_k (c({\tilde{\jmath}}_k^i)-c({\hat{\jmath}}_k^r),{\tilde{\jmath}}_k^i-{\hat{\jmath}}_k^r) \geq 0.
$$
This is true, since the cost $c(j)$ is increasing for $j>0$.
\end{enumerate}
%TODO: discuss monotonicity of the cost as an operator.
\begin{example}
If $c(j)=2^{1/3}|j|^{1/3}$, then from \eqref{revcost}, we have
$$
\sum_k (2^{1/3}|{\tilde{\jmath}}_k|^{1/3}- 2^{1/3}|{\hat{\jmath}}_k|^{1/3},
{\tilde{\jmath}}_k^i - {\hat{\jmath}}_k^i ) +
(2^{1/3}|-{\tilde{\jmath}}_k|^{1/3}- 2^{1/3}|-{\hat{\jmath}}_k|^{1/3},
{\tilde{\jmath}}_k^r - {\hat{\jmath}}_k^r) \geq 0.
$$
Which is
$$
\sum_k (2^{4/3}|{\tilde{\jmath}}_k|^{1/3}- 2^{4/3}|{\hat{\jmath}}_k|^{1/3},
{\tilde{\jmath}}_k^i - {\hat{\jmath}}_k^i + {\tilde{\jmath}}_k^r - {\hat{\jmath}}_k^r) \geq 0.
$$
\begin{equation}\label{expanded}
\sum_k (2^{4/3}|{\tilde{\jmath}}_k^i-{\tilde{\jmath}}_k^r|^{1/3}- 2^{4/3}|{\hat{\jmath}}_k^i-{\hat{\jmath}}_k^r|^{1/3},
{\tilde{\jmath}}_k^i - {\hat{\jmath}}_k^i +{\tilde{\jmath}}_k^r - {\hat{\jmath}}_k^r) \geq 0.
\end{equation}

This is true for all ${\tilde{\jmath}}_k^i , {\tilde{\jmath}}_k^r, {\hat{\jmath}}_k^i, {\hat{\jmath}}_k^r \geq 0.$

If ${\tilde{\jmath}}_k$ and ${\hat{\jmath}}_k$ satisfy the complementary condition, then we have the following cases
\begin{enumerate}
\item Case 1: ${\tilde{\jmath}}_k^r={\hat{\jmath}}_k^r=0$.
In this case, \eqref{expanded} becomes
$$
\sum_k (|{\tilde{\jmath}}_k^i|^{1/3}-|{\hat{\jmath}}_k^i|^{1/3},{\tilde{\jmath}}_k^i-{\hat{\jmath}}_k^i) \geq 0.
$$
\item Case 2: ${\tilde{\jmath}}_k^i={\hat{\jmath}}_k^i=0$.
In this case, \eqref{expanded} becomes
$$
\sum_k (|-{\tilde{\jmath}}_k^r|^{1/3}-|-{\hat{\jmath}}_k^r|^{1/3},{\tilde{\jmath}}_k^r-{\hat{\jmath}}_k^r) \geq 0.
$$
\item Case 3: ${\tilde{\jmath}}_k^i={\hat{\jmath}}_k^r=0$.
In this case, \eqref{expanded} becomes
$$
\sum_k (|-{\tilde{\jmath}}_k^r|^{1/3}-|{\hat{\jmath}}_k^i|^{1/3},{\tilde{\jmath}}_k^r-{\hat{\jmath}}_k^i) \geq 0.
$$
\item Case 4: ${\tilde{\jmath}}_k^r={\hat{\jmath}}_k^i=0$.
In this case, \eqref{expanded} becomes
$$
\sum_k (|{\tilde{\jmath}}_k^i|^{1/3}-|-{\hat{\jmath}}_k^r|^{1/3},{\tilde{\jmath}}_k^i-{\hat{\jmath}}_k^r) \geq 0.
$$
\end{enumerate}
\end{example}
\end{proof}
\begin{IMG}
{"1edge3", Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 0]],
Labeled[2 \[DirectedEdge] 3, Subscript["e", 1]],
Labeled[3 \[DirectedEdge] 4, Subscript["e", 2]],
Labeled[4 \[DirectedEdge] 5, Subscript["e", 3]],
Labeled[5 \[DirectedEdge] 6, Subscript["e", 4]]},
VertexLabels -> {1 -> Subscript["v",0], 2 -> Subscript["v", 1],
3 -> Subscript["v", 2],4 -> Subscript["v", 3],
5 -> Subscript["v", 4],6 -> Subscript["v", 5]},
EdgeStyle -> {1 \[DirectedEdge] 2 -> Dashed,
2 \[DirectedEdge] 3 -> Dashed,4 \[DirectedEdge] 5 -> Dashed,
5 \[DirectedEdge] 6 -> Dashed},
GraphLayout -> "RadialDrawing"](*\]\]\]\]\]\]\]\]\]*)}	
\end{IMG}
\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge3.pdf}
\caption{One edge network with transition edges.}
\end{figure}
\begin{IMG}
{"1edge4",
Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 0]],
Labeled[2 \[DirectedEdge] 3, Subscript["e", 1]],
Labeled[3 \[DirectedEdge] 4, Subscript["e", 2]],
Labeled[4 \[DirectedEdge] 5, Subscript["e", 3]],
Labeled[5 \[DirectedEdge] 6, Subscript["e", 4]],
Labeled[2 \[DirectedEdge] 1, Subscript["e", OverTilde[0]]],
Labeled[3 \[DirectedEdge] 2, Subscript["e", OverTilde[1]]],
Labeled[4 \[DirectedEdge] 3, Subscript["e", OverTilde[2]]],
Labeled[5 \[DirectedEdge] 4, Subscript["e", OverTilde[3]]],
Labeled[6 \[DirectedEdge] 5, Subscript["e", OverTilde[4]]]},
VertexLabels -> {1 -> Subscript["v", 0], 2 -> Subscript["v", 1],
3 -> Subscript["v", 2], 4 -> Subscript["v", 3],
5 -> Subscript["v", 4], 6 -> Subscript["v", 5]},
EdgeStyle -> {1 \[DirectedEdge] 2 -> Dashed,
2 \[DirectedEdge] 3 -> Dashed, 4 \[DirectedEdge] 5 -> Dashed,
5 \[DirectedEdge] 6 -> Dashed, 2 \[DirectedEdge] 1 -> Dashed,
3 \[DirectedEdge] 2 -> Dashed, 5 \[DirectedEdge] 4 -> Dashed,
6 \[DirectedEdge] 5 -> Dashed}, GraphLayout -> "RadialDrawing"](*\]\]\]\]\]\]\]\]\]\]\]\]\]\]\]\]\]\]*)}
\end{IMG}

\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge4.pdf}
\caption{One edge network with doubled edges.}
\end{figure}
\begin{example}
Consider example \ref{1edge}.
In order to transform it from the MFG setting to the Wardrop setting, we do the following.
\begin{itemize}
\item We add a transition edge between the entrance edge and the basic edge, we also add a transition edge between the basic edge and the exit edge.
So, we have $5$ edges and $6$ vertices.
\item We double the edges, so we get the extended network $\bar{\Gamma}$, which consists of $10$ edges and $6$ vertices.
%\item In each edge, we have a current.
%The currents in the doubled edges have an opposite direction.
%The currents in the transition edges are the transition currents in the MFG model.
\end{itemize}
\end{example}

%In the edge $e_k=(v_r,v_i)$, we have the complementary condition
%$$
%j_k^i >0 , \ u_k^r-u_k^i-c(j_k^i-j_k^r)=0
%$$
%$$
%j_k^i =0 , \ u_k^r-u_k^i-c(j_k^i-j_k^r) \geq 0
%$$
%In each edge of the new network, for every current we have
% $$
% j_{lr} \cdot (u_l-u_r-c_{rl})=0,
% $$
%with $j_{lr}=0$ if $u_l-u_r-c_{rl} > 0$.
%From the MFG, on every edge, we have a cost and a complementary condition
% $$
% j_{kl} \cdot (u_k-u_l-c_{kl})=0,
% $$
% and
%$$u_k-u_l-c_{kl} \geq 0.$$
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
\subsection{Recovering Mean-field games from Wardrop }\label{WtoMFg}
In this section, we show how to recover the MFG from the Wardrop model.
We start with a MFG problem and build the corresponding Wardrop problem.
We follow the same procedure in Section \ref{MFGtoW} to convert the MFG model into a Wardrop model, so that the structure of the network and the costs come from the MFG.
Then, we solve the new Wardrop problem, and we use its solution to recover the solution of the MFG, which consists of the currents $j$, and the value functions $u$.
The current in the MFG is the decomposition of the two currents in the new Wardrop.
The main issue is to define the value function.
For this, we present the following definition and result.
\begin{definition}
Given a Wardrop equilibrium, a \emph{regular vertex} is a vertex where some current $\tilde{\jmath} \neq 0$.
\end{definition}
\begin{lemma}\label{Lemma}
Suppose all loops have positive costs.
Given a regular vertex,
any path of positive currents leads to an exit.
In particular there is no current-carrying loops.
%there is at least one path through edges of positive currents, that connects the regular vertex to an exit vertex.
\end{lemma}
\begin{proof}
Consider a regular vertex, then at this vertex there are paths of positive currents.
These paths either end at an exit vertex or come back to the regular vertex.
Having these loops is incompatible with Wardrop equilibrium.
To prove this, for a loop of positive currents, consider the Wardrop equilibrium $\bm{{\tilde{\jmath}}^*}$ and take $\sigma >0$ small enough.
For the currents in each edge of the loop, we write
$${\hat{{\jmath}}}_k={{\tilde{\jmath}}^*}_k - \sigma.$$
Since the cost is positive, we have
\begin{equation}
\langle \tilde{c}({\bm{\tilde{\jmath}}}^*),{\bm{\tilde{\jmath}}}^*-({\bm{\tilde{\jmath}}}^*- \sigma) \rangle \geq 0.
\end{equation}
which contradicts the Wardrop equilibrium.
\end{proof}

Using Lemma \ref{Lemma}, we can connect any regular vertex to an exit vertex.
Hence, define
\begin{equation}\label{val}
\tilde{u}=\sum_k c_k({\tilde{\jmath}}_k)+ \bar{u},
\end{equation}
where $\tilde{u}$ is the candidate for the value function at the regular vertex, $c_k({\tilde{\jmath}}_k)$ is the cost in each edge of the path and $\bar{u}$ is the exit cost at the exit vertex.


\begin{proposition}\label{prop1}
The value function $\tilde{u}$ in \eqref{val} is well defined, i.e.
given a $\tilde{u}$ that has two different paths, the value function $\tilde{u}$ in these paths is the same.
Moreover, for any current carrying path and any other path, both going to the exit, the other path is at least as expensive.
\end{proposition}
\begin{proof}
Let $\tilde{u}$ be the value function at a regular vertex that has two outgoing paths, and let the first path be less expensive than the second path.
Consider the Wardrop equilibrium $\bm{{\tilde{\jmath}}^*}$ and take $\sigma >0$ small enough.
For the currents in each edge of the first path, we write
$${{\jmath}}^1_k={{\tilde{\jmath}}^*}_k+\sigma.$$
For the currents in each edge of the second path, we write
$${{\jmath}}^2_k={{\tilde{\jmath}}^*}_k-\sigma.$$
Since the new currents $\bm{{{\jmath}^1}}$ and $\bm{{{\jmath}^2}}$ satisfy Kirchhoff's law,
applying the definition of Wardrop equilibrium \eqref{Wardrop} on the second path, we get
\begin{equation}
\langle \tilde{c}({\bm{\tilde{\jmath}}}^*),{\bm{\tilde{\jmath}}}^*-({\bm{\tilde{\jmath}}}^*- \sigma) \rangle \geq 0.
\end{equation}
because the cost is positive, and this contradicts the Wardrop equilibrium.

Note that if the second path is not current carrying, the proof still holds and following the same steps we can prove that for any current carrying path and any other path, the other path is at least as expensive.
\end{proof}


%\begin{proposition}\label{prop2}
%For any current carrying path and any other path, both going to the exit, the other path is at least as expensive.
%\end{proposition}

%\begin{proof}
%The proof is similar to the previous proof.
%Consider the Wardrop equilibrium $\bm{{\tilde{\jmath}}^*}$ and take $\sigma >0$ small enough.
%For the currents in each edge of the current carrying path, we write
%$${{\jmath}^1}_k={{\tilde{\jmath}}^*}_k+\sigma.$$
%For the currents in each edge of the other path, we write
%$${{\jmath}^2}_k={{\tilde{\jmath}}^*}_k-\sigma.$$
%Since ${{\jmath}^1}_k$ and ${{\jmath}^2}_k$ satisfy Kirchhoff's law,
%Apply the definition of Wardrop equilibrium \eqref{Wardrop} on the other path, and since the cost is positive, we have
%\begin{equation}
% \langle \tilde{c}({\bm{\tilde{\jmath}}}^*),%{\bm{\tilde{\jmath}}}^*-({\bm{\tilde{\jmath}}}^*- \sigma) \rangle \geq 0.
%\end{equation}
%which contradicts the Wardrop equilibrium.
%\end{proof}
\begin{theorem}
The value function $\tilde{u}$ in the new Wardrop is the value function $u$ in the MFG.
\end{theorem}
\begin{proof}
The value function $u$ is the infimum among all paths.
Hence, by Proposition \ref{prop1}, $\tilde{u}$ is $u$.
\end{proof}
By this, we proved that we can recover the solution of a MFG problem by the solution of the corresponding Wardrop problem.

%There is also a variational description of Wardrop equilibrium when $c$ is monotone.
%Then,
%$$
%\min_{Aj=I} C(J)?+"<j,U_0>".
%$$
%This gives rise to a Lagrange multiplier $u$.
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}
{\color{green}
A natural question is which MFGs give rise to the particular cost structure of the Braess paradox? Or more generally to an
arbitrary cost $c(j)$? As we discuss in the following sections,
this question has several surprising answers.
In particular, we seek to address the following points: given an MFG, how do we recover the corresponding cost $c(j)$? Often, the interpretation of this cost is the travel time.
What are the travel times predicted by these MFGs? Can we calibrate the MFG so that the minimal cost is a given function $c(j)$? Can we do so in a way that $c(j)$ is also the travel time?

}
\begin{itemize}
\item Given a MFG problem on a network, we can build an extended oriented graph
\item On this oriented graph we have a "standard" wardrop equilibrium
\item The cost of this Wardrop equilibrium is "non-local" because of the graph is directed, introduces "clone" edges
\item When all costs are positive the situation is nicer (no loop type condition)
\item The uniqueness of wardrop is deduced from monotonicity conditions (this problem is also variational) - for this the cost depending on the current must be increasing.
\item  Monotonicity of the cost is not automatic for monotone MFGs nor it is a consequence of monotonicity of the MFG
\item When the cost is increasing, there is a convex variational formulation
\item Key issues: can we prove that monotone MFGs satisfy Wardrop monotonicity condition?
Also helpful is to show that certain non-monotone MFG will also satisfy Wardrop condition.
What is the relevance of the multiple MFG solutions for non-monotone MFG that satisfy the Wardrop monotonicity condition?
\end{itemize}


==> current-costs-backup.tex <==
\section{Wardrop equilibrium models and mean-field games}
\label{sec:current cost}





{\color{red}

What is the goal of this section: introduce the setting of generalized wardrop equilibrium; explain how this setting can be converted into a directed network by doubling edges.
Describe the inner product in a directed network.
Explain monotonicity conditons.
Define projection on affine subspace.
variational formulation and optimality conditions

}


Here, we discuss the connection between Wardrop equilibria and stationary congestion MFGs on networks.
Traditionally, the Wardrop equilibrium is formulated on a directed network.
In this network, agents seek to find the least costly path between entrances and exits.
In our Wardrop model, we consider the case where agents enter in a finite set of vertices with a prescribed current intensity and leave through a set of exit vertices where they pay an exit cost.
This problem is closely related to MFGs on networks, where the entry currents and the exit costs are similarly given.
However, in MFGs the network is not directed.
Thus, the direction of the current in each edge is not prescribed a priori.

We begin in Section \ref{Wmodel} with a discussion of the Wardrop equilibrium model and a uniqueness theorem.
Next, in Section \ref{MFG model} we present the MFG model.
Finally, in Section \ref{MFGtoW} we reformulate the MFG into a Wardrop model and make the connection between them.



\subsection{Wardrop equilibrium model}\label{Wmodel}


We consider a generalized Wardrop equilibrium for agents solving a minimal (travel) cost problem on a network.
This model consists of the following: 

\begin{enumerate}
  \item A finite \textbf{directed} network (graph), $\tilde{\Gamma}=(\tilde{E},\tilde{V})$, where
$\tilde{E} = \{ \tilde{e}_k : k \in \{1,2,\dots,\tilde{n}\} \}$ is the set of edges
and $\tilde{V}=\{\tilde{v}_i : i \in \{1,2,\dots, \tilde{m}\} \}$ is the set of vertices.
We write $\tilde{e}_k=(\tilde{v}_r,\tilde{v}_i)$.

  \item Agents enter the network through {\em entrance vertices} and exit it through {\em exit vertices} by choosing their paths in an optimal way, this is discussed next.
   
 \item   The \emph{current} or the flow is the number of agents crossing a given point per unit of time.
The current in the edge $\tilde{e}_k$ is denoted by $\tilde{\jmath}_k$.


 The current on the network is the $\tilde{n}$-dimensional vector $\bm{\tilde{\jmath}}=(\tilde{\jmath}_1,\dots,\tilde{\jmath}_{{\tilde{n}}})$.

   \item A flow of agents, the entry current $\iota >0$, is prescribed at entrance vertices.
   The entry currents in the other vertices are zero.
   This information is encoded in the $\tilde{m}$-dimensional vector $\tilde{B}$.
    At the exit vertices, the exit cost is zero.

 \item The \emph{travel cost} in each edge $\tilde{e}_k$ is given by the function $c_k(\bm{\tilde{\jmath}})$, this travel cost may be local, depends only on $\tilde{\jmath}_k$, or non local, depends on the whole vector $\bm{\tilde{\jmath}}$.
 
 We denote the vector of the costs in the edges by $c(\bm{\tilde{\jmath}})=(c_1(\bm{\tilde{\jmath}}),\dots,c_{\tilde{n}}(\bm{\tilde{\jmath}}))$.





\end{enumerate}

Define the $\tilde{m} \times \tilde{n}$ matrix $\tilde{K}$
%{\color{red}this is the \emph{incidence matrix} of the graph.
%We have to use auxiliary/virtual edges, these edges appear in the wardrop interpretation.}
\begin{equation}\label{K}
\tilde{K}_{ik}=
\begin{cases}
1 \ \ \text{if}  \ \tilde{e}_k=(\tilde{v}_i,\tilde{v}_r) \\ 
-1\ \ \text{if} \ \tilde{e}_k=(\tilde{v}_r,\tilde{v}_i)\\ 
0 \ \ \text{if} \  \tilde{v}_i \not\in \tilde{e}_k,
\end{cases}
\end{equation}  
%1 \ \ \text{if}  \ \tilde{e}_k \  \text{goes out of} \ \tilde{v}_i \\ 
%-1\ \ \text{if} \ \tilde{e}_k \  \text{goes into} \ \tilde{v}_i \\ 
%0 \ \ \text{if} \ \tilde{e}_k \  \text{is not incident to} \  \tilde{v}_i,
where $ i \in \{1,2,..., \tilde{m}\}$ and  $k \in  \{1,2,\dots,\tilde{n}\} $.
From definition, each row in $\tilde{K}$ corresponds to a vertex of the network and each column corresponds to an edge.

We say that a strategy ${\bm{\tilde{\jmath}}}$ is \emph{admissible} if $\tilde{K}\bm{\tilde{\jmath}}=\tilde{B}$, there $\tilde{m}$ equations account for splitting Kirchhoff's law and the boundary conditions.
Following Smith (\cite{Smith1979traffic}),  an admissible distribution of currents ${\bm{\tilde{\jmath}}}^*$, is a \emph{ Wardrop equilibrium} when no agent has a unilateral incentive to change its strategy.
Mathematically, this can be formulated  as follows, for any admissible 
 $\bm{\tilde{\jmath}}$, ${\bm{\tilde{\jmath}}}^*$ is a Wardrop equilibrium if
\begin{equation}\label{Wardrop}
 \langle c({\bm{\tilde{\jmath}}}^*),{\bm{\tilde{\jmath}}}^*-\bm{\tilde{\jmath}} \rangle \leq 0.
\end{equation}
The inner product in \eqref{Wardrop} is defined on the edges; that is, $\langle c,j \rangle = \sum_{k=1}^{\tilde{n}} c_kj_k $.

\begin{definition}
We say that $c$ is monotone if for any admissible ${\bm{\tilde{\jmath}}}$ and ${\bm{\hat{\jmath}}}$
\begin{equation}\label{mono}
 \langle c({\bm{\tilde{\jmath}}})-c({\bm{\hat{\jmath}}}),{\bm{\tilde{\jmath}}}-\bm{\hat{\jmath}} \rangle \geq 0.
\end{equation}
If for $\bm{\tilde{\jmath}} \neq \bm{\hat{\jmath}}$, the inequality in \eqref{mono} is strict, then we say that $c$ is strictly monotone.
\end{definition}


\begin{example}


If $c_k$ depends only on $\tilde{\jmath}_k$ and is increasing in  $\tilde{\jmath}_k$, then $c$ is monotone.


\end{example}


A \emph{current loop} is a nontrivial solution $\bm{\tilde{\jmath_0}} \geq 0$ of $\tilde{K}\bm{\tilde{\jmath_0}}=0$.
Given a solution of \eqref{Wardrop} $\bm{\tilde{\jmath^*}}$, for $\lambda \geq 0$ we have $\bm{\tilde{\jmath}}=\bm{\tilde{\jmath^*}}+\lambda \bm{\tilde{\jmath_0}}$ is also admissible. Thus, using this in \eqref{Wardrop}, we get 
$$
\langle c(\bm{\tilde{\jmath^*}}),\bm{\tilde{\jmath_0}} \rangle \geq 0. 
$$
This means that all current loops have non-negative costs. 
This is a necessary condition for the existence of the solutions. 
Strict positivity is necessary for strict monotonicity. 

Now, we state the uniqueness theorem for Wardrop equilibrium.

\begin{theorem}[Uniqueness of Wardrop equilibrium]
If the cost $c(\bm{\tilde{\jmath}})$ is strictly monotone on the set $\tilde{K}\bm{\tilde{\jmath}}={\tilde{B}}$, then there is at most one Wardrop equilibrium.
\end{theorem}

\begin{proof}
Suppose ${\bm{\tilde{\jmath}_1}} \neq{\bm{\tilde{\jmath}_2}}$ are two Wordrop equilibria.
Then, we have 
\begin{equation}
\left\langle c({\bm{\tilde{\jmath}_1}}),{\bm{\tilde{\jmath}_1}}-\bm{\tilde{\jmath}} \right\rangle \leq 0
\ \text{and} \ 
\langle c({\bm{\tilde{\jmath}_2}}),{\bm{\tilde{\jmath}_2}}-\bm{\tilde{\jmath}} \rangle \leq 0.
\end{equation}
Accordingly,
$$
\langle c({\bm{\tilde{\jmath}_1}})-c({\bm{\tilde{\jmath}_2}}),{\bm{\tilde{\jmath}_1}}-{\bm{\tilde{\jmath}_2}} \rangle \leq 0,
$$
which contradicts the strict monotonicity of $c$.


\end{proof}


%%%%%%%%%%%%%%%%

\subsection{MFG problem in a single edge}\label{cost}

Now, we study the MFG problem and the travel cost in a single edge. 



 \subsubsection{MFG system in an edge}
 In each edge $e_k$, which we identify with the interval $[0,1]$, we have the following MFG system, (for simplicity, we omit the dependence of $u$, $m$, and $j$ in the edge index $k$)
 
 
 \begin{equation}\label{MFGgeneral}
  \begin{cases}
    H(x,u_x(x),m(x))=0 \\ 
    \left(-m(x)D_pH(x,u_x(x),m(x)\right)_x=0,
  \end{cases}
\end{equation}
where $m$ is the population density and $u$ is the value function.
The first equation is the Hamilton-Jacobi (HJ) equation and the second is the transport equation.
From the second equation in \eqref{MFGgeneral}, the current $j=-mD_pH$ is constant.
%This system is supplemented by boundary conditions which we discuss below.

\begin{example}
Let 
$$
H(x,p,m)=\frac{|p|^2}{2m^{\alpha}} + V(x) - g(m),
$$
where $g$ is an increasing function, $V$ is a smooth function and $0\leq \alpha \leq 2$ is the congestion strength.
Then, \eqref{MFGgeneral} becomes
\begin{equation}\label{mfgs}
  \begin{cases}
    \frac{|u_x|^2}{2m^{\alpha}} + V(x) = g(m)\\
    (-m^{1-\alpha}u_x)_x=0,
  \end{cases}
\end{equation}
There are two special values of the parameter $\alpha$,  
$\alpha=0$ for the uncongested MFG and  $\alpha=1$, corresponds to the critical congestion model, for which the system decouples.  
  Using the fact that the current, $j=-m^{1-\alpha}u_x$, is constant in the edges, we transform the MFG system in the edges into the following algebraic system %for $j>0$
\begin{equation}\label{current mfg}
\begin{cases}
\frac{j^2}{2m^{2-{\alpha}}}+V(x)=g(m)\\
j\int_0^1m^{\alpha-1}dx=u(0)-u(1),\\
\end{cases}
\end{equation}
provided $m>0$.
Notice that sometimes we will refer to the last equation in \eqref{current mfg} by \emph{edge equation}.
When $j>0$, the second equation in \eqref{current mfg} determines $u(0)$ as a function of $u(1)$, whereas when $j<0$, this equation determines $u(1)$ as a function of $u(0)$. This has to do with how boundary conditions are specified and we will discuss this next.  

\end{example}

\subsubsection{Travel cost in an edge}

In our MFG the cost in the edge depends only on the current in this edge.
In each edge, which is identified by $[0,1]$. $j>0$ corresponds to traveling from $0$ to $1$ (left to right). Similarly, $j<0$ corresponds to traveling from $1$ to $0$ (right to left).
In each edge, we have two costs. The cost of moving from left to right or from $0$ to $1$, and it is denoted by $c_{01}(j)$. The cost of moving from left to right or from $1$ to $0$ and it is denoted by $c_{10}(j)$. 

In the MFG, the boundary conditions that we choose need to be consistent with the current in the edge, in the following way
\begin{equation}\label{BC}
\begin{cases}
j>0 \Rightarrow u(0)=c_{01}(j)+u(1), \\ 
j<0 \Rightarrow u(1)=c_{10}(j)+u(0).
\end{cases}
\end{equation}
 Agents at a given vertex always have the possibility of moving to the opposite vertex, even if this is suboptimal.  This is written as
\begin{equation}\label{optforc}
\begin{cases}
u(1)\leq c_{10}(j)+u(0), \\ 
u(0)\leq c_{01}(j)+u(1).
\end{cases}
\end{equation}

%When the current is zero, we do not have equalities just inequalities. 


\begin{proposition}
If the costs in \eqref{optforc} are positive ,then the inequalities in \eqref{optforc} are redundant.
% and there is a compact way to write this. 
\end{proposition}

\begin{proof}

\eqref{optforc} implies, 
$$
-c_{01}(j) \leq u(1)-u(0) \leq c_{10}(j).
$$
If $j \neq 0$, one of the two inequalities is an equality.
%$$
%j>0 \Rightarrow \  u(1)=c_{10}(j)+u(0), \\ 
%$$
%and
%$$
%j<0 \Rightarrow \ u(0)=c_{01}(j)+u(1).
%$$
Since the costs are positive, then the other inequality holds.   
If the cost is allowed to be negative this can cause existence issues. 

\end{proof}

Now, we show how to define the cost in the edge. 
Consider an edge with positive current, $j>0$. This means that $u$ has a Dirichlet boundary condition to the right (at 1).
First, by the fundamental theorem of calculus, we note that 
$$
u(0)=u(1)-\int_0^1{u_x} dx.
$$
Thus $-u_x$ can be represented as a cost per unit of length. 
So, it is natural to define 
$$
c_{01}(x,j)=-p(x,j),
$$
where $p(x,j)$ solves 
\begin{equation}\label{mfgsys}
\begin{cases}
H(p(x,j),m(x,j),x)=0, \\
-m(x,j)D_pH(p(x,j),m(x,j),x)=j.
\end{cases}
\end{equation}
Consequently, 
$$
u(0)=u(1)+ c_{01}(j), 
$$
where
$$
c_{01}(j)=\int_0^1 c_{01}(x,j).
$$


The computation of the cost can be further analyzed as follows.
The current is $j=-mD_pH(x,u_x,m)$, thus 
$$
D_pH(x,u_x,m)=-\frac{j}{m}.
$$
If $H$ is strictly convex in $p$ then 
$ p \rightarrow D_pH(x,p,m)$
is invertible. Therefore, we can write 
\begin{equation}\label{ux}
u_x=D_pH(x,p,m)^{-1}(-\frac{j}{m}) = -D_vL(x,-\frac{j}{m},m),
\end{equation}
where $L$ is the Legendre transform of $H$
$$
L(x,v,m)= \sup_p \ [-pv-H(x,p,m)].
$$
Using \eqref{ux} in the HJ equation, we obtain 
$$
H(x,-D_vL(x,-\frac{j}{m}),m)=0,
$$
the preceding equation determines $m$ as a function of $j$ and $x$. 
Then, we have an optimal cost of traveling from vertex $0$ to $1$ with a trajectory $x(t)$ 
$$
c_{01}(j)=\int_0^T L(x,\dot{x},m(x,j)) dt, 
$$ 
where $x(0)=0$ and $x(T)=1$.

Then, this is the same (provided $\dot{x}>0$) and parametrizing the velocity by $x$,
$$
\dot{x}=v(x,j), \ dx=\dot{x}dt
$$

\begin{equation}\label{Lv}
c_{01}(j)=\int_0^1 \frac{L(x,v(x,j),m(x,j))}{v(x,j)} dx.
\end{equation}



If we want to minimize this (for $v(x,j)>0$ it may be that the infimum is achieved for $v(x,j)=0$), 
\begin{equation}\label{L/v}
-\frac{L(x,v(x,j),m(x,j))}{v(x,j)^2}+\frac{D_vL(x,v(x,j),m(x,j))}{v(x,j)}=0,
\end{equation}
this is the Euler-Lagrange equation for \eqref{Lv}, and we can write it  
$$
D_vL(x,v(x,j),m(x,j))=\frac{L(x,v(x,j),m(x,j))}{v(x,j)}.
$$
This determines $v$ as function of $x$. Then, along an optimal trajectory the cost 
$$
c_{01}(j)=\int_0^1 D_vL(x,v(x,j),m(x,j)). 
$$
(This is the best we can do when traveling possibly in the wrong direction). 


\begin{proposition}
If $L(x,0,m)>0$ and coercive, then there exists a function $v(x,j)>0$ solving \eqref{L/v}. Moreover, if $L(x,v,m)$ is strictly convex, then $v(x,j)$ is unique. 
\end{proposition}

\begin{proof}
\eqref{L/v} is the necessary optimality condition for 
$$\min_{v>0} \frac{L(x,v,m)}{v(x,j)},$$
and 
$$ \lim_{v \rightarrow 0} \frac{L(x,v,m)}{v(x,j)}= +\infty. $$
By coercivity, we have 
$$ \lim_{v \rightarrow \infty} \frac{L(x,v,m)}{v(x,j)}= +\infty. $$
Then, there exists a minimizer $v(x,j)>0$, which is a critical point for \eqref{L/v}.
Uniqueness of $v(x,j)$ follows from 
 $D^2_{vv}L(x,v,m) >0 $ for $v(x,j)>0$ and $L(x,0,m)>0$.
 
\end{proof}


%(we may need $L(x,0,m)>0$ to prevent $v(x)=0$ )

When $j>0$, we know a bit more because
$$
v(x,j)=-D_pH(x,u_x,m(x,j))
$$
and $v(x,j)=\frac{j}{m(x,j)}$. 
Then, we just have to compute 
$$
c_{01}(j)=\int_0^1 D_vL(x,\frac{j}{m(x,j)},m(x,j)). 
$$

\begin{example}[Reversible Hamiltonian]

Suppose the Hamiltonian is 
$$
H=\frac{p^2}{2}-m.
$$
Then, the Lagrangian is 
$$
L=\frac{v^2}{2}+m.
$$
The MFG system is 
\begin{equation*}
\begin{cases}
\frac{u_x^2}{2}=m\\
-(mu_x)_x=0.
\end{cases}
\end{equation*}
The cost is
$$
c(j)=\int_0^1 D_vL(x,v(x),m(x,j)) dx.
$$
where $m(x,j)$ is obtained by replacing $u_x$ by $\frac{-j}{m}$ in the HJ equation 

$$
\frac{1}{2}(\frac{j}{m})^2=m,
$$
hence
$$
m(x,j)=(\frac{j^2}{2})^{1/3}.
$$
The formula $vD_vL=L$ implies
$$
v(x,j)=(2m(x,j))^{1/2}.
$$
Substituting $m(x,j)$ in the previous identity, we get 

$$
v(x,j)=(2(\frac{j^2}{2})^{1/3})^{1/2}.
$$
Then, the final formula for the cost is 
$$
c_{01}(j)=\int_0^1 2^{1/3} |j|^{1/3} dx =  2^{1/3}|j|^{1/3}.
$$


This cost actually independent on the sign of $j$ because the Lagrangian is reversible. 
We can see this by using the other formula for $j>0$
$$
c_{01}(j)=\int_0^1 \frac{j}{m(x,j)} = \frac{j}{(j^2/2)^{1/3}}=(2j)^\frac{1}{3}.
$$


\end{example}


\begin{proposition}
If the Hamiltonian is reversible $(H(-p)=H(p))$, then the cost is reversible i.e. $c_{01}(j)=c_{10}(j)$.
%This means that the cost for traveling along an edge from right to left is the same as the cost for traveling from left to right along the same edge. 
\end{proposition}

\begin{proof}
Since $H$ is reversible, 
$$
H(-p)=H(p) \Rightarrow L(-v)=L(v).
$$
$m$ is given by solving \eqref{mfgsys}. 
For $j>0$, traveling from $0$ to $1$, the optimal velocity is $v=\frac{j}{m}$, which solves the necessary optimality condition \eqref{L/v}. 
For same $j$ and $m$, we look at the optimal trajectory connecting $1$ to $0$. We claim that the velocity $-v(x,j)$ is optimal. This is true because $-v(x,j)$ also solves \eqref{L/v}.
Then by \eqref{cost}, we have 
$$c_{01}(j)=c_{10}(j).$$
Thus, the cost is reversible. 
\end{proof}


%reversibility implies also, 
%$$m(x,j)=m(x,-j).$$
%$$c_{01}(j)=c_{01}(-j).$$
%Perhaps, for some cases we have  $m(x,j)=m(x,-j).$, without reversibility. 


{\color{red}
\begin{example}[Non-reversible Hamiltonian] 


\end{example}

}

\paragraph{ Monotonicity of the cost }
Now, we examine the monotonicity properties of the cost. Assuming $j>0$, and differentiating \eqref{mfgsys} with respect to $j$, we get

\begin{equation}\label{dj}
\begin{aligned}
& -D_pH(-c(x,j),m(x,j),x) \frac{\partial c(x,j)}{\partial j}+D_mH(-c(x,j),m(x,j),x) \frac{\partial m(x,j)}{\partial j}=0, \\
& m(x,j)D_{pp}H(-c(x,j),m(x,j),x)\frac{\partial c(x,j)}{\partial j} \\
& -(D_pH(-c(x,j),m(x,j),x)+m(x,j)D^2_{pm}H(-c(x,j),m(x,j),x)\frac{\partial m(x,j)}{\partial j}=1.
\end{aligned}
\end{equation}
From the first equation, we have

\begin{equation}
\frac{\partial c(x,j)}{\partial j}=- \frac{m(x,j)D_mH(-c(x,j),m(x,j),x)}{j}\frac{\partial m(x,j)}{\partial j}.
\end{equation}
Thus, if $D_mH(p(x),m(x,j),x) \leq 0$, then $m(x,j)$ and $c(x,j)$ have the same monotonicity with respect to $j$ and opposite otherwise.

The solution of \eqref{dj} is 

\begin{gather}\label{djsol}
 \begin{bmatrix} 
 \frac{\partial c}{\partial j} \\
 \frac{\partial m}{\partial j} 
  \end{bmatrix}
 =
 \frac{1}{(D_pH)^2+mD_pHD_{pm}^2H-D_mHD_{pp}^2Hm}
  \begin{bmatrix}
  -D_mH \\
  -D_pH
   \end{bmatrix}.
\end{gather}

\begin{result}
For general MFGs of the form \eqref{MFGgeneral}, Lions \cite{cursolions}\cite{porreta} introduced a condition on $H$ that gives the uniqueness of solution in a number of cases.
This condition is that the matrix 
\begin{gather}
 \begin{bmatrix}
  -\frac{2}{m}D_mH & D_{pm}H \\
  D_{pm}H &  2D^2_{pp}H
   \end{bmatrix}.
  \end{gather} 
is non-negative definite.
\end{result}

Lions condition implies 
$$
\frac{\partial c}{\partial j} \geq 0,
$$
%because the denominator in \eqref{djsol} is the determinant of the matrix.
However, Lions condition is not necessary.
We show that in the next example for separable Hamiltonians.


\begin{example}
Suppose $H$ is separable, i.e.
\[
D^2_{pm}H=0\  \text{and} \ D_mH=-g^{\prime}(m).
\]
From \eqref{djsol}, we get
\begin{equation}\label{dc1}
\frac{\partial c}{\partial j}=\frac{g^{\prime}(m)}{(D_pH)^2+D_{pp}Hmg^{\prime}(m)}.
\end{equation}
If $g^{\prime}(m) >0$ then $\frac{\partial c}{\partial j} \geq 0$.
When $g^{\prime}(m) <0$, the analysis is more delicate.

Consider the case where 
\[
H(p,m)=\frac{|p|^\gamma}{\gamma}-g(m).
\]
Then, the HJ equation becomes
$$\frac{|p|^\gamma}{\gamma}=g(m),$$
and we have
\begin{equation*}
\begin{aligned}
& D_pH  = p|p|^{\gamma -2}, \\
& (D_pH)^2=|p|^{2(\gamma -2)}=(\gamma g(m))^{2-\frac{2}{\gamma}}, \\
& D^2_{pp}H= (\gamma-1)|p|^{\gamma -2}=
(\gamma-1)(\gamma g(m))^{1-\frac{2}{\gamma}}.
\end{aligned}
\end{equation*}
%\begin{equation*}
%\begin{aligned}
%& D_pH  = p|p|^{\gamma -2}, \\
%& (D_pH)^2=p^2|p|^{2(\gamma -2)}=(\gamma g(m))^{\frac{2}{\gamma}}(\gamma g(m))^{2-\frac{4}{\gamma}}, \\
%& D^2_{pp}H= |p|^{\gamma -2}+(\gamma-2)p^2|p|^{\gamma -4}=
%(\gamma g(m))^{1-\frac{2}{\gamma}}+(\gamma-2)(\gamma g(m))^{\frac{2}{\gamma}}(\gamma g(m))^{1-\frac{4}{\gamma}}.
%\end{aligned}
%\end{equation*}
Substituting in \eqref{dc1}, we get
 \begin{equation}
 \frac{\partial c}{\partial j}=\frac{g^{\prime}(m)}{(\gamma g(m))^{2-\frac{2}{\gamma}}+(\gamma-1)(\gamma g(m))^{1-\frac{2}{\gamma}}mg^{\prime}(m)}.
 \end{equation}
 Thus, to get $\frac{\partial c}{\partial j} \geq 0$ when $g^{\prime}(m) <0$, we need 
\begin{equation}\label{cond}
 \gamma g(m) +(\gamma -1)m g^{\prime}(m) \leq 0.
\end{equation}
In the case of a power this condition holds.

Now, consider 
 $$g(m)=m^{-\beta}, \ \beta>0,$$ 
 then \eqref{cond} becomes
$$\gamma-(\gamma-1)\beta \leq 0. $$
Hence, for 
 $\beta \geq \frac{\gamma}{\gamma-1}, $ 
 we have $\frac{\partial c}{\partial j} \geq 0$. 


\end{example}
 
\subsubsection{Relevance and interpretation of the results}
Crowd aversion is Lions monotonicity condition, i.e.
both $c$ and $m$ increase with $j$.
It is possible, however, to have a crowd seeking behavior, i.e.
$g$ decreasing with $c$ increasing in $j$ but in this case $m$ decreases with $j$.

This is actually something that happens in uncongested highways. As speed increases, cars increase their distances, hence density decreases. 
Let us look at the velocity
$$ \frac{j}{m}= v(j), $$
This is the optimal velocity at which the agents move. 
What happens to the velocity as function of $j$ ? 
\begin{equation*}
\frac{\partial}{\partial j}\left[v(j)\right]=
\frac{\partial}{\partial j} \left(\frac{j}{m} \right)= \frac{1}{m} - \frac{j}{m^2} \frac{\partial m}{\partial j}.
\end{equation*}
From \eqref{djsol} and using that $v(j)=-D_pH$, we have 
$$
\frac{\partial m}{\partial j}= \frac{-D_pH}{M} =\frac{j}{m M},
$$
where $M=(D_pH)^2+mD_pHD_{pm}^2H-D_{pp}^2HD_mHm$. Hence
$$
\frac{\partial}{\partial j}\left[v(j)\right]=
\frac{1}{m}\left[ 1-\frac{j^2}{m^2}\frac{1}{M} \right]=
-\frac{1}{m} \frac{mvD^2_{pm}H+D^2_{pp}HD_mHm}{M}.
$$
In the separable case, we have  
$$
\frac{\partial}{\partial j}\left[v(j)\right]=-\frac{1}{m}\frac{D^2_{pp}Hg^{\prime}(m)m}{M}. 
$$
So, if reverse Lions condition holds
$$
\frac{\partial v}{\partial j} \geq 0. 
$$
Another quantity of interest, $\frac{\partial m}{\partial v}, \geq 0$ which means uncongested model. 
In the separable case, we have 
$$
\frac{\partial m}{\partial v}= -\frac{v}{D^2_{pp}Hg^{\prime}(m)m}. 
$$
If $g^{\prime}$ increasing, $m$ decreases with $v$. Whereas if $g^{\prime}$ decreasing, $m$ increases with $v$. This is independent on $m$. 

{\color{red}
\paragraph{Recovering $m$ from $j$}
Solving the first equation in \eqref{mfgsys} for $m$ and substituting in the second equation + solvability conditions.} 




%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Mean-field game model on a network}\label{MFG model}

Now, we examine the MFG formulation on networks. 
Our MFG model consists of the following

\begin{enumerate}
  \item A finite \textbf{undirected} network, $\Gamma=(E,V)$, where
$E = \{e_k : k \in \{1,2,...,n\} \}$ is the set of edges
and $V=\{v_i : i \in \{1,2,..., m\} \}$ is the set of vertices.
We write $e_k=(v_r,v_i)$.

  \item Agents enter the network through {\em entrance vertices} and exit it through {\em exit vertices}. To every entrance vertex, $v_i$, we associate an auxiliary edge, $e_k=(v_r,v_i)$, called the {\em entrance edge}.
Similarly, to every exit vertex, $v_i$, we associate an auxiliary edge, $e_l=(v_i,v_s)$, called {\em exit edge}.

Sometimes, the original edges of the network will be called basic edges, to distinguish between them and the auxiliary edges.
  
 \item  A flow of agents, the entry current $\iota >0$, is prescribed at entrance vertices.
  The entry currents in the other vertices are zero.
   This information is encoded in the $m$-dimensional vector $B$.
  At the exit vertices, the exit cost $\bar{u}$ is given.
 
 \item For moving from $e_k$ to $e_l$ through a common vertex, agents pay a \emph{switching cost}, $\psi_{kl}$.
 Often, we may require $\psi_{kl} \geq 0$.

\item  For any vertex, $v_i$, that has more than two incident edges, we require the following triangle-type inequality in the switching costs, 
\[
\psi_{kl} \leq \psi_{km}+ \psi_{ml}.
\]

\item The switching cost from an entry edge to a basic edge is $0$, and from a basic edge to an entry edge is $\infty$. Similarly, the switching cost from an exit edge to a basic edge is $\infty$, and from a basic edge to an exit edge is $0$.

Remark:


\begin{remark} this avoids entry through exits and exit through entrances. 
\end{remark}
 \end{enumerate}
 
 


    
   On the network $\Gamma$, we define the following variables 
       

\begin{itemize}

\item \textbf{Edge currents:}  The \emph{current} $j_k$ in the edge $e_k=(v_r,v_i)$ is decomposed in positive and negative parts, $j_k= j_k^i-j_k^r$ such that 
  \begin{equation}\label{js}
 j^i_k,j^r_k \geq 0 \ \text{and} \ j_k^i \cdot j^r_k=0.
  \end{equation}
 where $j^i_k$ is the current going to the vertex $v_i$ and $j^r_k $ is the current going to the vertex $v_r$.
 This means that all agents in an edge move in the same direction.

\item \textbf{Transition currents:}
The \emph {transition current} from $e_k$ to $e_l$ through a common vertex is denoted by $j_{kl}$.
The transition currents also satisfy
\begin{equation}\label{jts}
j_{kl},j_{lk}\geq 0 \ \text{and} \ j_{kl} \cdot j_{lk}=0.
\end{equation}


\item \textbf{Value functions:}
The \emph{value function} in the edge $e_k=(v_r,v_i)$ at the vertex $v_i$ is denoted by $u_k^i$.


\item \textbf{Travel costs:}
In the edge $e_k=(v_r,v_i)$, the cost of moving from $v_r$ to $v_i$ is $c_{ri}(j_k)$, and the cost of moving from $v_i$ to $v_r$ is $c_{ir}(j_k)$. 


\end{itemize}

These variables are related to each other through the following equations and inequalities

\paragraph*{\textbf{Optimality conditions at the vertices}}
In the process of minimizing their travel cost, agents choose the least expensive path.
They decide to switch from $e_k$ to $e_l$ through the common vertex $v_i$, if 
\begin{equation}\label{optcond}
  u^i_k\leq  \min\limits_{l \in \mathcal{K}} \big\{ u_l^i + \psi_{kl}  \big\}.
\end{equation} 


\paragraph*{\textbf{Complementarity conditions at the vertices}}
If the transition current $j_{kl}$ is not zero, then the agents are moving from $e_k$ to $e_l$ through $v_i$.
This implies that $u_k^i+ \psi_{kl}=u_l^i$.
So, we have the following, 
\begin{equation}\label{ujcomp}
 j_{kl} \cdot (u^i_l +\psi_{kl}- u^i_k)=0, \ \forall i, k, l.
\end{equation}

\paragraph*{\textbf{Optimality conditions in the edges}}
In the edge $e_k=(v_r,v_i)$, for any $j_k$ we have 
\begin{equation}\label{optcond2}
\begin{cases}
  u^r_k \leq   c_{ri}(j_k) + u_k^i, \\
  u^i_k \leq   c_{ir}(j_k) + u^r_k.
 \end{cases}
\end{equation} 
For $j_k>0$, \eqref{optcond2} becomes
$$
 u^r_k =  c_{ri}(j_k^i) + u_k^i .
 $$
For $j_k<0$, \eqref{optcond2} becomes
$$
u_k^i=  u^r_k  + c_{ir}(-j_k^r).
$$

The costs $c_{ri}(j_k^i)$ and $c_{ir}(-j_k^r)$ may not be the same, unless the system is reversible.



\paragraph*{\textbf{Complementarity conditions in the edges}}
In the edge $e_k=(v_r,v_i)$, we have the complementary conditions
$$
j_k^i \cdot (u_k^r-u_k^i-c_{ri}(j_k))=0,
$$
which can be written in the following way
$$
j_k^i >0 \Rightarrow \  u_k^r-u_k^i-c_{ri}(j_k)=0,
$$
or
$$
j_k^i =0 \Rightarrow \  u_k^r-u_k^i-c_{ri}(j_k) \geq 0.
$$
 

 


\paragraph*{\textbf{Balance equations}}
For the edge $e_l=(v_i,v_s)$, the current $j_l^i$ is equal to the sum of the transition currents from $e_l$ to all the other incident edges at $v_i$, this models a splitting of the current.
\begin{equation}\label{balance1}
   \sum_k j_{lk}=j^i_l.
\end{equation} 
We have a similar equation for the gathering of the transition currents, the current $j_l^s$ is the sum of the transition currents from all the incident edges at $v_i$ to $e_l$.
\begin{equation}\label{balance2}
   \sum_k j_{kl}= j^s_l.
\end{equation} 

If $j_{kl} > 0 $, then $u$ has Dirichlet boundary condition at $1$ for the HJ equation.
The gathering condition on the other side determines the boundary condition at the left for the transport equation.

 \paragraph*{\textbf{Entry edge equations}} 
 In every entry edge $e_k=(v_r,v_i)$, given the entering current $\iota_i$ at the entrance vertex $v_i$, we have 
 \begin{equation}\label{incondj}
 \begin{cases}
j^i_k=\iota_i.\\
j^r_k=0.
\end{cases}
\end{equation}
In $e_k$, we also, have
\begin{equation}\label{incondu}
u^r_k=u^i_k.
\end{equation}

\paragraph*{\textbf{Exit edge equations}} 
In every exit edge $e_l=(v_i,v_s)$, given the exit cost $\bar{u}$ at the exit vertex $v_i$, we have 
\begin{equation}\label{outcondu}
u^s_l = u^i_l = \bar{u}(v_i).
\end{equation}
In $e_l$, we also have
\begin{equation}\label{outcondj}
j^i_l=0.
\end{equation}

\paragraph*{\textbf{Basic edge equation}}
In the each basic edge, we have 
\begin{equation}\label{edgeeq}
j\int_0^1m^{\alpha-1}dx=u(0)-u(1).
\end{equation}
or
$$
(j_k^i-j_k^r) \int_0^1m_k^{\alpha-1}dx=u_k^r-u_k^i.
$$

%$u(0)-u(1)=c(j_k^i-j_k^r)\sgn(j_k^i-j_k^r).$
 

Now, we present a simple example to illustrate this framework. 

\begin{IMG}
{"1edge", Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 1]]}, 
 VertexLabels -> {1 -> Subscript["v", 1], 2 -> Subscript["v", 2]}, GraphLayout -> "RadialDrawing"](*\]*)}	
\end{IMG}

\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge.pdf}
\caption{Simple network with one edge.}
\end{figure}


\begin{IMG}
{"1edge2", Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 0]], 
  Labeled[2 \[DirectedEdge] 3, Subscript["e", 1]],
  Labeled[3 \[DirectedEdge] 4, Subscript["e", 2]]}, 
 VertexLabels -> {1 -> Subscript["v",0], 2 -> Subscript["v", 1], 
   3 -> Subscript["v", 2],4 -> Subscript["v", 3]}, 
   EdgeStyle -> {1 \[DirectedEdge] 2 -> Dashed, 
  3 \[DirectedEdge] 4 -> Dashed},
  GraphLayout -> "RadialDrawing"](*\]*)}	
\end{IMG}

\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge2.pdf}
\caption{One edge network with entrance and exit edges.}
\end{figure}

\begin{example}\label{1edge}
Consider a network of one edge, $e_1=(v_1,v_2)$. Given an entry current $\iota$ at the entrance vertex $v_1$, and the exit cost $\bar{u}$ at the exit vertex $v_2$. Assuming $e_{0}=(v_0,v_1)$ is the entrance edge and $e_2=(v_2,v_3)$ is the exit edge. For simplicity we set all the switching costs to zero. We consider the MFG \eqref{mfgs} and write the corresponding equations in the critical congestion case, i.e. $\alpha=1$. 

\begin{itemize}



\item 
\eqref{js} gives
\begin{equation*}
\begin{cases}
j_0^1 \cdot j_0^0 =0, \ j_0^1,j_0^0 \geq 0, \\ 
j_1^2 \cdot j_1^1 =0, \ j_1^2,j_1^1 \geq 0, \\
j_2^3 \cdot j_2^2 =0, \ j_2^3,j_2^2 \geq 0.
\end{cases}
\end{equation*}


\item 
\eqref{optcond} gives
\begin{equation*}
\begin{cases}
u_0^1 \leq u_1^1, \ u_1^1 \leq u_0^1, \\
u_1^2 \leq u_2^2, \ u_2^2 \leq u_1^2. 
\end{cases}
\end{equation*}

Which implies $u_0^1 = u_1^1$ and $u_1^2= u_2^2$. 



\item  
\eqref{jts} gives 
\begin{equation*}
\begin{cases}
j_{01} \cdot j_{10} =0, \ j_{01},j_{10} \geq 0, \\ 
j_{12} \cdot j_{21} =0, \  j_{12},j_{21} \geq 0. 
\end{cases}
\end{equation*}


\item 
\eqref{balance1} and \eqref{balance2} give 

\begin{equation*}
\begin{cases}
j_0^1=j_{01}, \ j_0^0=j_{10}, \\
j_1^2=j_{12}, \ j_1^1=j_{10}, \\ 
j_1^2=j_{01}, \ j_1^1=j_{21}, \\
j_2^3=j_{12}, \ j_2^2=j_{21}. 
\end{cases}
\end{equation*}



\item \eqref{incondj} and \eqref{incondu} give
\begin{equation*}
\begin{cases}
j_0^1= \iota, \ j_0^0=0, \\
u_0^0= u_0^1.
\end{cases}
\end{equation*}

\item \eqref{outcondj} and \eqref{outcondu} give
\begin{equation*}
\begin{cases}
u_2^2 =u_2^3= \bar{u},\\
j_2^2 = 0. 
\end{cases}
\end{equation*}



\item
\eqref{ujcomp} give 
\begin{equation*}
\begin{cases}
j_{10} \cdot (u_0^1 - u_1^1)=0, \ j_{01} \cdot (u_1^1 - u_0^1)=0, \\
j_{21} \cdot (u_1^2 - u_2^2)=0, \  j_{12} \cdot (u_2^2 - u_1^2)=0. 
\end{cases}
\end{equation*}

\item The last equation in \eqref{current mfg} gives the edge equation

$$
u_1^1-u_1^2= j_1^2-j_1^1.
$$

\end{itemize}


\end{example}





%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%







\subsection{Reformulation of mean-field game as Wardrop equilibrium}\label{MFGtoW}

Now, we explain how to reformulate the MFG model in Section \ref{MFG model} as a Wardrop model as the one described in Section \ref{Wmodel}. We then, show that given the MFG, we have a Wardrop equilibrium. For this, we identify the network, the currents and the costs in the Wardrop equilibrium.

 In Wardrop equilibrium, the network $\tilde{\Gamma}$ is directed but in MFG the network $\Gamma$ is undirected.
In $\Gamma$, we double the undirected edges so that every edge is directed,  and we blow-up the connecting vertices into a set of pairs of auxiliary edges we will call them \emph{transition edges}.
Now, we have an extended directed network $\bar{\Gamma}$ for the MFG model. In this new network, we have the following 

\begin{itemize}

\item Every current $j_k^i$ or transition current $j_{kl}$, corresponds to a directed edge in $\bar{\Gamma}$.

\item  The transition currents are edge currents in the transition edges. 

\item We consider the matrix $K$ that represents the equations \eqref{balance1}, \eqref{balance2}, \eqref{incondj} and \eqref{outcondj}. Each column corresponds to a current and hence to an edge. Each row corresponds to a vertex. 

\item Some currents in this network will appear in two rows of $K$. These two rows give the two vertices of the corresponding edge. 

\item Some appear only once. These are the exit vertices and we simply add a vertex which is a sink and hence there is no need for a further balance equation there. 


\item Balance equations are equivalent to Kirchhoff's law in the Wardrop setting.

\item The switching costs $\psi_{kl}$ turn into travel costs in the transition edges.

\item To make the exit cost $\bar{u}$ at the exit vertex $v_i$ zero, we add an auxiliary edge $e_k=(v_i,v_r)$ incident to $v_i$ such that the exit cost at $v_r$ is zero and in the auxiliary edge the cost is $c(j_k^i)=j_k^i\cdot\bar{u}$.


\end{itemize}

\begin{proposition}
If the cost is monotone in Wardrop, then the cost in MFGs is monotone. 
\end{proposition}



\begin{proof}
Let $\hat{c}(j)=c_{01}(j)-c_{10}(j)$. By the monotonicity of $\hat{c}$ in Wardrop, we have 
$$
 \langle \hat{c}({\bm{\tilde{\jmath}}})-\hat{c}({\bm{\hat{\jmath}}}),{\bm{\tilde{\jmath}}}-\bm{\hat{\jmath}} \rangle \geq 0.
$$
Then, 
$$
 \langle c_{01}({\bm{\tilde{\jmath}}})-c_{10}(-{\bm{\tilde{\jmath}}}),{\bm{\tilde{\jmath}}}-\bm{\hat{\jmath}} \rangle 
 -  \langle c_{01}({\bm{\hat{\jmath}}})-c_{10}(-{\bm{\hat{\jmath}}}),{\bm{\tilde{\jmath}}}-\bm{\hat{\jmath}} \rangle 
 \geq 0.
$$
Finally, we have 
\begin{align*}
 \langle  c_{01}({\bm{\tilde{\jmath}}}_{01}-{\bm{\tilde{\jmath}}}_{10})-
 c_{01}({\bm{\hat{\jmath}}}_{01}-{\bm{\hat{\jmath}}}_{10}),
 ({\bm{\tilde{\jmath}}}_{01}-{\bm{\tilde{\jmath}}}_{10})-({\bm{\hat{\jmath}}}_{01}-{\bm{\hat{\jmath}}}_{10})  \rangle \\
 + 
 \langle  c_{10} ({\bm{\tilde{\jmath}}}_{01}-{\bm{\tilde{\jmath}}}_{10})-
 c_{10}({\bm{\hat{\jmath}}}_{01}-{\bm{\hat{\jmath}}}_{10}),
 ({\bm{\tilde{\jmath}}}_{01}-{\bm{\tilde{\jmath}}}_{10})-({\bm{\hat{\jmath}}}_{01}-{\bm{\hat{\jmath}}}_{10})   \rangle
 \geq 0.
\end{align*}
Thus, the cost in the MFG is monotone. 
\end{proof}

{\color{red}
Q: What about $\hat{c}(0)$? }


\begin{theorem}
If $j^*$ is a solution to the MFG system, then it is also a Wardrop equilibrium. 
\end{theorem}

\begin{proof}

For admissible $j^*$ and $j$, we have 

$$
Kj^*=B \ \text{and} \ Kj=B.
$$

$$
K(j^*-j)=0
$$

$$
u^{T}K(j^*-j)=0
$$

each current appears twice, one for each of its vertices but with different signs.
The previous computation yield 
$$
\sum (u_k^r-u_k^i)(j^{i*}_k-j_k^i)
$$

If $j^{i*}_k >0$, $u_k^r-u_k^i=c(j_k^i-j_k^r)$. 
If $j^{i*}_k =0$, $u_k^r-u_k^i \geq c(j_k^i-j_k^r)$. 
$$
\langle c, j^*-j \rangle \geq 0
$$
This is Wardrop equilibrium. 

\end{proof}



\begin{IMG}
{"1edge3", Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 0]], 
  Labeled[2 \[DirectedEdge] 3, Subscript["e", 1]],
  Labeled[3 \[DirectedEdge] 4, Subscript["e", 2]],
  Labeled[4 \[DirectedEdge] 5, Subscript["e", 3]], 
  Labeled[5 \[DirectedEdge] 6, Subscript["e", 4]]}, 
 VertexLabels -> {1 -> Subscript["v",0], 2 -> Subscript["v", 1], 
   3 -> Subscript["v", 2],4 -> Subscript["v", 3],
   5 -> Subscript["v", 4],6 -> Subscript["v", 5]}, 
   EdgeStyle -> {1 \[DirectedEdge] 2 -> Dashed, 
  2 \[DirectedEdge] 3 -> Dashed,4 \[DirectedEdge] 5 -> Dashed, 
  5 \[DirectedEdge] 6 -> Dashed},
  GraphLayout -> "RadialDrawing"](*\]*)}	
\end{IMG}

\begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge3.pdf}
\caption{One edge network with transition edges.}
\end{figure}

\begin{IMG}
{"1edge4",
Graph[{Labeled[1 \[DirectedEdge] 2, Subscript["e", 0]],
  Labeled[2 \[DirectedEdge] 3, Subscript["e", 1]],
  Labeled[3 \[DirectedEdge] 4, Subscript["e", 2]],
  Labeled[4 \[DirectedEdge] 5, Subscript["e", 3]],
  Labeled[5 \[DirectedEdge] 6, Subscript["e", 4]],
  Labeled[8 \[DirectedEdge] 7, Subscript["e", OverTilde[0]]], 
  Labeled[9 \[DirectedEdge] 8, Subscript["e", OverTilde[1]]], 
  Labeled[10 \[DirectedEdge] 9, Subscript["e", OverTilde[2]]], 
  Labeled[11 \[DirectedEdge] 10, Subscript["e", OverTilde[3]]], 
  Labeled[12 \[DirectedEdge] 11, Subscript["e", OverTilde[4]]]}, 
 VertexLabels -> {1 -> Subscript["v", 0], 2 -> Subscript["v", 1], 
   3 -> Subscript["v", 2], 4 -> Subscript["v", 3], 
   5 -> Subscript["v", 4], 6 -> Subscript["v", 5], 
   7 -> Subscript["v", OverTilde[0]], 
   8 -> Subscript["v", OverTilde[1]], 
   9 -> Subscript["v", OverTilde[2]], 
   10 -> Subscript["v", OverTilde[3]], 
   11 -> Subscript["v", OverTilde[4]], 
   12 -> Subscript["v", OverTilde[5]]}, 
 EdgeStyle -> {1 \[DirectedEdge] 2 -> Dashed, 
   2 \[DirectedEdge] 3 -> Dashed, 4 \[DirectedEdge] 5 -> Dashed, 
   5 \[DirectedEdge] 6 -> Dashed, 8 \[DirectedEdge] 7 -> Dashed, 
   9 \[DirectedEdge] 8 -> Dashed, 11 \[DirectedEdge] 10 -> Dashed, 
   12 \[DirectedEdge] 11 -> Dashed}, GraphLayout -> "RadialDrawing"](*\]*)}
   \end{IMG}

  \begin{figure}[ht]
\centering
\includegraphics[scale=1]{figures/1edge4.pdf}
\caption{One edge network with doubled edges.}
\end{figure}
 
   

\begin{example}
Consider example \ref{1edge}.  In order to transform it from the MFG setting to the Wardrop setting, we do the following. 

\begin{itemize}

\item We add a transition edge between the entrance edge and the basic edge, we also add a transition edge between the basic edge and the exit edge. So, now we have $5$ edges and $6$ vertices. 

\item We double the edges, so we get the extended network $\bar{\Gamma}$, which consists of  $10$ edges and $12$ vertices. 

\item In each edge, we have a current. The currents in the doubled edges have an opposite direction. The currents in the transition edges are the transition currents in the MFG model. 

 
\end{itemize}



\end{example}


% \paragraph{The costs} In the undirected edge $e_k=(v_r,v_i)$, based on the discussion in Section \ref{cost}, the cost is $c(j_k^i-j_k^r)$ and the edge equation becomes
%$$
%u(0)-u(1)=c(j_k^i-j_k^r)\sgn(j_k^i-j_k^r). 
%$$
%If we double $e_k$ to make it direct, we get the edge $e_{\tilde{k}}=(v_{\tilde{r}},v_{\tilde{i}})$. The cost in $e_k$ in this case is, 
%\begin{equation*}
%c_k(j_k^i,j_k^r)= 
%\begin{cases}
%+\infty \ \text{if} \ j_k^i \neq 0 \  \text{and} \ j_k^r \neq 0, \\
%c(j_k^i) \ \text{otherwise}. 
%\end{cases}
%\end{equation*}
%Similarly, we define the cost in $e_{\tilde{k}}$. This enforces the complementary condition.  


%In the edge $e_k=(v_r,v_i)$, we have the complementary condition
%$$
%j_k^i >0 , \  u_k^r-u_k^i-c(j_k^i-j_k^r)=0
%$$
%$$
%j_k^i =0 , \  u_k^r-u_k^i-c(j_k^i-j_k^r) \geq 0
%$$

%In each edge of the new network, for every current we have 
 % $$
 % j_{lr} \cdot (u_l-u_r-c_{rl})=0, 
 % $$
%with $j_{lr}=0$ if $u_l-u_r-c_{rl} > 0$. 

%From the MFG, on every edge, we have a cost and a complementary condition
%  $$
%  j_{kl} \cdot (u_k-u_l-c_{kl})=0, 
% $$
%  and
%$$u_k-u_l-c_{kl} \geq 0.$$


%%%%%%%%%%%%%%%%

\subsection{Recovering Mean-field games from Wardrop }

We have a cost on each edge that we know how to compute and then we have all the inequalities for MFGs.

\textbf{Claim:} An MFG solution is a Wardrop equilibrium in the previous sense.

There is also a variational description of Wardrop equilibrium when $c$ is monotone.
Then, 
$$
\min_{Aj=I} C(J)?+"<j,U_0>".
$$
This gives rise to a Lagrange multiplier $u$.

\textbf{Question:} what is the connection between $u$ and the solution? (they are the same).



%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}


{\color{green}
A natural question is which MFGs give rise to the particular cost structure of the Braess paradox? Or more generally to an 
arbitrary cost $c(j)$? As we discuss in the following sections, 
this question has several surprising answers.
In particular, we seek to address the following points: given an MFG, how do we recover the corresponding cost $c(j)$? Often, the interpretation of this cost is the travel time.
What are the travel times predicted by these MFGs? Can we calibrate the MFG so that the minimal cost is a given function $c(j)$? Can we do so in a way that $c(j)$ is also the travel time? 

}


\begin{itemize}
\item Given a MFG problem on a network, we can build an extended oriented graph
\item On this oriented graph we have a "standard" wardrop equilibrium
\item The cost of this wardop equilibrium is "non-local" because of the orientedness of the graph introduces "clone" edges
\item When all costs are positive the situation is nicer (no loop type condition)
\item The uniqueness of wardrop is deduced from monotonicity conditions (this problem is also variational) - for this the cost depending on the current must be increasing.
\item Increasingness of the cost is not automatic for monotone MFGs nor it is a consequence of monotonicity of the MFG
\item When the cost is increasing, there is a convex variational formulation

\item Key issues: can we prove that monotone MFGs satisfy Wardrop monotonicity condition?
Also helpful is to show that certian non-monotone MFG will also satisfy Wardrop condition.
 What is the relevance of the multiple MFG solutions for non-monotone MFG that satisfy the wardorp monotonicity condition?

\end{itemize}




==> stationary-mfg.tex <==
\section{Stationary mean-field games on networks}
\label{sec:smfg on networks}



%$$u_k^i-u_k^r= c_k(j_k^r-j_k^i) \cdot \text{sgn}(j_k^r-j_k^i).$$

Thus the MFG can be converted into a minimal travel cost problem, such as the one addressed in Section \ref{sec:current cost}.
Now, we illustrate this concept by computing $c$ in the following example.
\begin{example}
  Suppose $q>1$, $A>0$, $\alpha\geq 0$, $r>0$, $V\equiv 0$, 
  and 
   $g(m) = B m^r$.
   Consider the Lagrangian, 
   $
   \mathcal{L}(v,m) = A m^\alpha \frac{|v|^q}{q}+B m^r
   $, with Hamiltonian $\mathcal{H}(p,m) =  A m^\alpha \frac{|p/(A m^\alpha)|^{q'} }{q'} - B m^r$,
          where $1/q+1/{q'}=1$. 
        
  For this Hamiltonian,  \eqref{mfgs} becomes 
  \begin{equation}\label{eq: mfg conjugate}
  \begin{cases}
  (A m^\alpha)^{1-q'} \frac{|u_x|^{q'} }{q'} = B m^r\\
   \left(-m (Am^{\alpha})^{1-q'}\sgn (u_x)\left|u_x\right|^{q'-1}\right)_x=0.
  \end{cases}
\end{equation}
We will convert the MFG \eqref{eq: mfg conjugate} into a minimal travel cost problem. 
The last equation in \eqref{eq: mfg conjugate} gives that $j= -m (Am^{\alpha})^{1-q'}\sgn (u_x)\left|u_x\right|^{q'-1}$ is constant.
  Assuming $j>0$ and $\alpha \neq 1${\color{red}(why?)}, we get 
  $u_x = -A j^\frac{1}{q'-1}  m^{\alpha -\frac{1}{q'-1}}$.
  Substituting $u_x$ in the first equation in \eqref{eq: mfg conjugate} and integrating $u_x$, we get 
  \begin{equation}\label{current mfg2}
  \begin{cases}
    \frac{1}{q'}A m^{\alpha-\frac{q'}{q'-1}}  j^{\frac{q'}{q'-1}} = B m^r \\
      m > 0\\
      A j^\frac{1}{q'-1}  \int_0^1m^{\alpha -\frac{1}{q'-1}}dx =u(0)-u(1).\\
    \end{cases}  
\end{equation}
Solving the first equation in \eqref{current mfg2} for $m$, we obtain
\begin{align*}
  m &= \left(\frac{A}{B q'}\right)^{\frac{q'-1}{(r-\alpha)(q'-1)+q'}}j^{\frac{q'}{(r-\alpha)(q'-1)+q'}}.
\end{align*}
  Using this expression in the last equation of  \eqref{current mfg2}, we get 
 \begin{align}
  \label{eq: homo power}
  u(0)-u(1) = 
  C_{\alpha, q, r, A,B} j^{\theta(\alpha, q, r)},
\end{align} 
where 
\begin{align*}
\theta(\alpha, q, r) &= \frac{\alpha -\alpha  q'-r}{\alpha  \left(q'-1\right)-(r+1)
q'+r}\\ 
C_{\alpha, q, r, A,B} &=A^{\frac{(r+1) \left(q'-1\right)}{\alpha -\alpha  q'+r
q'+q'-r}}\left(B q'\right)^{\frac{\alpha +\alpha  \left(-q'\right)+1}{\alpha -\alpha  q'+r
q'+q'-r}}  .
\end{align*}
 
The formula \eqref{eq: homo power} shows that the family of Lagrangians introduced in this example produces costs that are powers of the  current. Although the above  family of MFGs is quite general, all of them give $c(0)= 0$, unless $c$ is constant.
This last case only happens if $\alpha-\alpha q'-r=0$.
\end{example}



Thus, this example raises the following question - given a travel cost $c(j)$ which MFGs correspond to this travel cost? 
We address this question in the next section.

